Maxmin convolutional neural networks for image classification

Convolutional neural networks (CNN) are widely used in computer vision, especially in image classification. However, the way in which information and invariance properties are encoded through in deep CNN architectures is still an open question. In this paper, we propose to modify the standard convo- lutional block of CNN in order to transfer more information layer after layer while keeping some invariance within the net- work. Our main idea is to exploit both positive and negative high scores obtained in the convolution maps. This behav- ior is obtained by modifying the traditional activation func- tion step before pooling. We are doubling the maps with spe- cific activations functions, called MaxMin strategy, in order to achieve our pipeline. Extensive experiments on two classical datasets, MNIST and CIFAR-10, show that our deep MaxMin convolutional net outperforms standard CNN.

==> images/schema2pdf <==
%PDF-1.5
%âãÏÓ
1 0 obj
<</Metadata 2 0 R/Pages 3 0 R/Type/Catalog>>
endobj
2 0 obj
<</Length 61591/Subtype/XML/Type/Metadata>>stream
<?xpacket begin="" id="W5M0MpCehiHzreSzNTczkc9d"?>
<x:xmpmeta xmlns:x="adobe:ns:meta/" x:xmptk="Adobe XMP Core 5.6-c067 79.157747, 2015/03/30-23:40:42        ">
   <rdf:RDF xmlns:rdf="http://www.w3.org/1999/02/22-rdf-syntax-ns#">
      <rdf:Description rdf:about=""
            xmlns:dc="http://purl.org/dc/elements/1.1/"
            xmlns:xmp="http://ns.adobe.com/xap/1.0/"
            xmlns:xmpGImg="http://ns.adobe.com/xap/1.0/g/img/"
            xmlns:xmpMM="http://ns.adobe.com/xap/1.0/mm/"
            xmlns:stRef="http://ns.adobe.com/xap/1.0/sType/ResourceRef#"
            xmlns:stEvt="http://ns.adobe.com/xap/1.0/sType/ResourceEvent#"
            xmlns:stMfs="http://ns.adobe.com/xap/1.0/sType/ManifestItem#"
            xmlns:illustrator="http://ns.adobe.com/illustrator/1.0/"
            xmlns:xmpTPg="http://ns.adobe.com/xap/1.0/t/pg/"
            xmlns:stDim="http://ns.adobe.com/xap/1.0/sType/Dimensions#"
            xmlns:stFnt="http://ns.adobe.com/xap/1.0/sType/Font#"
            xmlns:xmpG="http://ns.adobe.com/xap/1.0/g/"
            xmlns:pdf="http://ns.adobe.com/pdf/1.3/">
         <dc:format>application/pdf</dc:format>
         <dc:title>
            <rdf:Alt>
               <rdf:li xml:lang="x-default">Impression</rdf:li>
            </rdf:Alt>
         </dc:title>
         <xmp:MetadataDate>2016-02-01T15:24:45+01:00</xmp:MetadataDate>
         <xmp:ModifyDate>2016-02-01T15:24:45+01:00</xmp:ModifyDate>
         <xmp:CreateDate>2016-02-01T15:23:16+01:00</xmp:CreateDate>
         <xmp:CreatorTool>Adobe Illustrator CC 2015 (Macintosh)</xmp:CreatorTool>
         <xmp:Thumbnails>
            <rdf:Alt>
               <rdf:li rdf:parseType="Resource">
                  <xmpGImg:width>256</xmpGImg:width>
                  <xmpGImg:height>92</xmpGImg:height>
                  <xmpGImg:format>JPEG</xmpGImg:format>
                  <xmpGImg:image>/9j/4AAQSkZJRgABAgEASABIAAD/7QAsUGhvdG9zaG9wIDMuMAA4QklNA+0AAAAAABAASAAAAAEA&#xA;AQBIAAAAAQAB/+4ADkFkb2JlAGTAAAAAAf/bAIQABgQEBAUEBgUFBgkGBQYJCwgGBggLDAoKCwoK&#xA;DBAMDAwMDAwQDA4PEA8ODBMTFBQTExwbGxscHx8fHx8fHx8fHwEHBwcNDA0YEBAYGhURFRofHx8f&#xA;Hx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8f/8AAEQgAXAEAAwER&#xA;AAIRAQMRAf/EAaIAAAAHAQEBAQEAAAAAAAAAAAQFAwIGAQAHCAkKCwEAAgIDAQEBAQEAAAAAAAAA&#xA;AQACAwQFBgcICQoLEAACAQMDAgQCBgcDBAIGAnMBAgMRBAAFIRIxQVEGE2EicYEUMpGhBxWxQiPB&#xA;UtHhMxZi8CRygvElQzRTkqKyY3PCNUQnk6OzNhdUZHTD0uIIJoMJChgZhJRFRqS0VtNVKBry4/PE&#xA;1OT0ZXWFlaW1xdXl9WZ2hpamtsbW5vY3R1dnd4eXp7fH1+f3OEhYaHiImKi4yNjo+Ck5SVlpeYmZ&#xA;qbnJ2en5KjpKWmp6ipqqusra6voRAAICAQIDBQUEBQYECAMDbQEAAhEDBCESMUEFURNhIgZxgZEy&#xA;obHwFMHR4SNCFVJicvEzJDRDghaSUyWiY7LCB3PSNeJEgxdUkwgJChgZJjZFGidkdFU38qOzwygp&#xA;0+PzhJSktMTU5PRldYWVpbXF1eX1RlZmdoaWprbG1ub2R1dnd4eXp7fH1+f3OEhYaHiImKi4yNjo&#xA;+DlJWWl5iZmpucnZ6fkqOkpaanqKmqq6ytrq+v/aAAwDAQACEQMRAD8A9U4q7FXYq7FXYq7FXYqo&#xA;XEt0skKQQiQO9JpGYKsaDcnuzE9AAPnTASejKIG9ljPm3zD5c8rwR/pxLnUE1J2IRws61ioaem7J&#xA;GgHIU4rv333www8W3Nq1GujhAlI8PTb8Wx7/AJXJ+Xnqwzfo649W3UJbyfV4OUagUCofUqo37ZZ+&#xA;WPc4X8t4aI4jv72h+cP5chJoxpk4juDyuE+rQUkINauPU+Lfxx/KnuCf5bw7es7e9x/OL8uiIAdM&#xA;uCLU1th9Wg/dGoNY/wB58O4HTH8qe5H8t4d/Wd+fNHaL+Z3kXVtXSwtdPmS71NvRkkkt4QJOQ3Er&#xA;B2LA+9cEtORZIbcPauPJIQjI305pzPdWUmpaXpdto8ctiLy5trktbc0tzDA06yKY1aKMO/EcnIqT&#xA;SlemNjlCY2GwJHxBo/a5/iTBuzZ82QfUYhcyXKPKs0q8GpI5QdByETExBvhG/HLOHe0cZqvx8+ak&#xA;Tq0FtGAsV9OGpK1Tb1TxC0lBbx3UfLpg9QHen0E/zR8/1K31ib6y0P1WX01XkLisXpsafZA586/N&#xA;aZK9+THhFXf3qf165+ret+j7j1OXH6vyt/UpT7VfV4U/2VfbBxGuTLgF1Y+39Sp9Zm+sRxfVZeDr&#xA;yaesXBDQ/Cw5867fsqR74b8mPCKu/vWC9uTDLJ9QnDxkBIuUHKQE0qv73jTv8RGDiPcngF8x9v6l&#xA;xupw0AFnMRKAZGBhpFXs9ZKmn+RyxvyXhG+4+39TX1u4rP8A6FN+5/uzWH97/wAY/wB5t/s+ONnu&#xA;XhG24+3b7GjeXASFvqM5Mpo6coKxb0q/7yh8fhLY8R7l4BvuPt/Uv+szfWJIvqsvBF5LPWLg5oPh&#xA;Uc+dd/2lA98N+SOEVd/epm+uRbCb9H3BkLcTbhrf1AKfaJ9XhT/ZV9sHEa5MuAXVj7f1Kv1iX616&#xA;P1aT06V+s1j9OtOlOfqf8Jhvfkx4RV38FIXtyYHl/R84dW4rAWg5sP5lPq8KfNgcHEe5lwC6sfb+&#xA;pf8AWZ/ViT6pLxkUM8tYuMZ/lf8Aecq/6oIxvyRwiuY+39SxdQ5LO31aceh2KbvuR+73+LpjxeSf&#xA;D5bjdd+kIgIOcU6NcGiL6MjFTUD94UVlTr1YjHiRwHflt5u/SFsGnVvUQWylpXeKRE4jclXZQjf7&#xA;EnHiC+GdvNWhmhniSaCRZYZAGjkQhlYHoQRsRhBtiQQaK/Ch2KuxV2KuxV2KuxVA6UtpILi/ty7f&#xA;XZS5d6dIwIl4UH2KR8l+de+QhXMdW3LYqJ6f2vMf+cgv95tE/wBe4/VHmXpvqdB27/dD+t+gvnjz&#xA;DJqMMq/V6lW32zb4zcduaOxo4ZwPFXEmekC4Nqsk9ebDocrzEXTqe0zAZDGHJH5S61kf5c/8pzov&#xA;/MSv6jlOf6C7Dsn/ABiPx+4voDynJ6h1o+GqXK/8CEH8M1OnhwxI/pS+2RL2GOfEPifsKfZezdir&#xA;sVdirAdR/K/UbrUb69j8x3MP6SvI7y5hCHgDA/7lYwkkf2IljT95zUleXHoFxpYCTz5u0h2jGMRH&#xA;gHpjQ+PPp32dq7rULf8AKvWYLOeGLzNMstw8sryhLggSSSxTI4VrtjzRom+MsWPL7Qpg/Ln+cyl2&#xA;lAkE4xtXd3EfzfP3bKtz+WvmK4ilifzbd8JygljYTunprC8LRKr3LDi/Op5ciaAklviwnBI/xfj5&#xA;sY9oYwb8Mbe7vv8Am/j3bI/zJ+X1xrV8036ZuLW0ksmsp7GL1FjkrG6B5AksYbiZK8WH68M8BJ59&#xA;GvBrhjFcIJ4rv8BAp+XmpPcXEB823gpNBN9Vt5rmExW6h19Pit18Al8VCr8PwqAKAeBL+cWf8oQ/&#xA;1OPLrwnfv+n7/mtvfy18zXbMz+b7qvwGJeNxwR0jRfUCrdKCxeLlvsKniA3xYnBI/wAX4+bKHaGO&#xA;P+TH2f8AE/j3bI//AABqE1jqFnfa9c3UWoWjWboxm9NOSxhWRWnc/DwetW5MGo7NSpPgne5NX52I&#xA;kDGAHCb6fq/srYIV/wAt9a428MXmq+htYLcxFEe5DtJT4X5LcqAqv8QXjWnw8uACgeBL+cWf5+G5&#xA;OONk+X/E/jnzR+oeTvMM8WlLa+ZJ7d9OiSOZ2WZ/rDoPtyBbiMNzNOfPkdtitSTI4pGvVya4arGO&#xA;K4A8R8tvs+6m5vJGpS6DYaW3mG+E1rcm4ur9JbhJrhWZj6RZZg6rRgKcqCnTHwjQHEgayImZcEdx&#xA;QFCh9iVN+WvmWQwtN5uuXkg+tNE5jlNJbiFoYpQGuWAeHnUU+H+UKSWMfAPWRbx2hjF1jG9d3Q2R&#xA;9PX8XyZT5S0CfQdDh02e9fUZ42d5b2UFXkaRy5ZqtISxJ3PLfLccOEVzcLVZxlmZAcI7k4yxx0Iq&#xA;Tw6gKPEthLHxSCgVxcBmclKD4uaklt9uNe5yPI+TZYMf6X6EXkmt2KuxV2KuxVCTanbQ6pa6awb6&#xA;xdxTTRED4ONuYw/I9j++WmKovFWFS/mZp2n6tb+XruxvJNZ+pyXEkUMSIryW8LSPFbpNJFJMz8Cs&#xA;XpKyua8WPCTgI3W7KdcRrk81/Nnzrb+YJrSySzns5bH98FuKK7R3MSGjpXlHJHNHJE6HuuxNdsnT&#xA;fU6Ptz+6H9b9BedSxJIAHFab5nRkQ81jymB2RFratPIsUdAx2AynNlEImR5MNyfMplceWb+3Rnen&#xA;wU5jeo5Cor9Ga7D2zhySAHXk5WfQZsUeKQ2Rv5dinnrRh1pcr+o5sM30Ft7J/wAYj8fuL3LyXcSi&#xA;LWykLTD9NX6ngVBHGQAfbK5gmNPVaT6T/Wn/ALosjGoWlQHf0WOyiYNFU/5PMLy+jA5KIxVbLKkU&#xA;Zkc0UeG5JOwAHck7AYq8o/NTz15t8vaxaW+n3a28c9v6zxelFJxJdlpyZWPRd/fL8OMSu3U9p66e&#xA;Ax4a3vn8Hn8v57edIn4SaqoY9vq8H/NGZY0NtGPU6yYuMY1+PNERfnP59lXkmpKR/wAw8H/NGQlp&#xA;QObiZO1tRA0RH8fFf/yuH8wf+riv/IiD/mjI/l4tf8t5u6Py/ay38svzC82a35ri0/U7wT2zQyu0&#xA;YiiT4lFRuiqfxynLiERYdp2fr55Z8Eq5X9zPfJ9kJDc6/JcSTXeqKkMysIlQLZyTJGyiNEbkyv8A&#xA;EWJ6ClMwNJklPFGUvqMQS7k10ZJmQh2KqVxMyBUjAaeTaNT026sf8le/3d8VfPU/5vef0nkRdRXi&#xA;rED9xB0B/wBTMyOCJFvMZ+2M0ZyiOGgSPxup/wDK4fzA/wCriv8AyIg/5ow/l4tX8t5u6Py/a7/l&#xA;cP5gf9XFf+REH/NGP5eK/wAt5u6Py/a2Pzg/MEn/AI6K/wDIiD/mjE6eKY9s5yaAj+Pi9N/L/wA1&#xA;61rFlpMuoXRlkupbxZKJGgcQqhQEKopx5E7U981OqyShnxwH0yu/hGw9Ho8/iYhI8z+gshsNLGie&#xA;V9Ntb+U38mkLCPrUStEWKH0/U4tJKR8DHlVzUVy6dVZczFZNDq8s/PqSRfMtgFYgfUgaAkf7tfM3&#xA;TgG7ec7byyiYcJI58vgwC30rzBcwrPbWd3PC9eEsccjqaGhoygjqMry67S45GM544yHQyiD8nVY4&#xA;auY4ojIR3jiKFlN3DK0UxkjlQlXjfkrKR1BB3BzKhwTiJRoxPIholnzRNGUgR5lZ683+/G+85PgH&#xA;cx/M5f50vmWYflJLK35haUGdiP8ASNiT/wAs0uVZogROzn9l58ktREGRI36+Re3+VbXTLrSNN1A2&#xA;kJubYTraT+mnOJZZCJBG1KoH4DlTrTfNB2SJDTREiSd+f9YvWjJx7p/mxSg9H+rjSrRLeUzQxRLE&#xA;krAgt6Y4VIO4Pw5GFUKbMt8Rvm8q/wCcjGkXTtHMa83Dz0Qs6V/uv2kV2H0DLsfN12uEeEWLF+W2&#xA;3P1UHhs0t79ZCrcRKgaRnX1FDemvFa09NqfEfo8d+Iv4pd4dQcOnq/DnZ8pfrH45d662u7+3uoLj&#xA;9IQikioB8IVmM3MKoIqWaKqfb+iu+QyRM4mJIooOPDGj4WS+fy79+9mOp+bku4LiKK6Msl0ysYTI&#xA;GWP00WM8FH2e1f7c0vZ/Y0ceUE16L95s3v3r2hrs2TCImJiOuy78uf8AlOdG/wCYlf1HOhz/AEFw&#xA;eyf8Yj8fuL3L8u25W/mA+GvakPumpmLlG49w+567DGh8T95ZYQCCCKg7EHKm1DHT7RRWIG3pvWFj&#xA;GtfEqPgP+yBxVAaDp97DE73t/LqIM8s1rJMqIVWViwACAfCgbjHWp49+wVeR/n3/AMpNp/8AzBD/&#xA;AJOyZl6bq8529zh8f0PEtY0E3N4sqMQCenvmzhIEb9G3s3tYY8XDLondtAIIFiG/EbnKJy4jboNR&#xA;mOSZkVYfCK9+39crO+yI+gcXXp+v9TOvyV/5TqH/AIwTf8RynU/S7TsP++P9X9Ieyfl8/qeT9Of+&#xA;YSH75nzXYocMBHuD0mmnxY4nviGRZY3LJpkijLtU02CjqSdgB7nFVlvCylpZaGeSnKm4UDog9h+P&#xA;XFXyRdf71Tf67frzZQ+kPB6r+9n/AFj96nk3HdvgSA2fhFO56/0wDdtl6Rw9ev6v1vXvywl4xeVE&#xA;/wB+XGqj7oUOazVY7yg936no+z8lY8I7+P8AS9cvhdGyuBZkLdmNxbs32RJxPAnY7csErrbm72FW&#xA;L5PBfzn1nR9X16xudKvrfULdLURvNaypMgcSM3EtGWFeLA098zNN1ea7e5w+P6En8oedH0Gxv7Yo&#xA;ZfVX1LQbcVnpxPIbEqRQnf8AZ980nbns+Ndlxzvh4dpd5jz28xv0/ivpTV2V2udLCcau94/1uX43&#xA;6ebGJZZJZHllcySyEs7sSWZiakknqTnRwgIgRiKA5B0spGRJJslrif8AM48QZ+DLy+Y/WzD8ogf+&#xA;VhaSaf8ALR/1DS5VmkDAuw7MxSjqY2O/7i9p/LSb1vJOmy/zet+FxIM12PHwR4XoOzJmWCJPn95Z&#xA;Pk3PQtl66y3UTwLFEkpa3dAAHWRQ7MRX7XqM3Lx698jHqznVA3+P7Hk3/OR63J0/RBbAF/VnJUkr&#xA;VQIyQGG4J6Vy7GCTs4GtyY4Q9ZoHbv8AseES2l56VDaJd3IQIZJiAr0VHJI5HiPVQUoO1KAfFlvB&#xA;Ludd+bwnfxCADyAHn/RspitlbKQVUjiwYfE3VTUE775eMUe51OTtHMSQJWPcOXyVI7WCLeNaFjyO&#xA;5O4qO58DjHGAWOo1mWcQJHYjy7/2Bk/5c/8AKcaN/wAxK/qOOf6Cy7J/xiPx+4vU/Lfmm18v+XPN&#xA;mp3EbSra65rMtN0jpFc0IeYj04/tbcjU/sgnbMTKbI9w+57QinpeVIef/mx531byymlpYRQSpemb&#xA;11uFdgRD6dF+B02PqHl4/fl2HGJXbqu09dPT8PCBvfPyphsX52ee5RWPTrFh7RT/APVbDMYo/VKn&#xA;Vx7bznlGJ+B/WxDzn5q1jzLfw3mqQQwTQReiqwK6rxDFtw7Oa1bL8Ij/AAm3B1eunnI4gBw9zH8v&#xA;cNHaLbRXepQWstAkrEFj22JzB7RzyxYZTjzi36XEMmSMTyLJvN3ljS9It0kiYOWHSvfOc7C7Zz6q&#xA;ZjIO17Y7OhgAMTuVf8lf+U7h/wCME3/Ec6nU/Sw7D/vj/V/SHrv5Xvz8haO380TH/ko2YuQVIh6L&#xA;SCsMB/RH3MpyDkPMvN35uHy/5pu9LfSfrn1P0/Sk+semP3kSyE8PSff4+Na9PmcyIYOIXbpdX2v4&#xA;OQw4brz8r7ku/wCV/wAlK/4eNP8AmKP/AFQw+AP5zj/y/wD0P9l+x49MxeV3IpzYtTwqa5lRFB0O&#xA;XJxzMu8krck1sq8maJp2syzpcUh+rqDyJ+0Wr8ulM5f2g7SzaQRMN+K+nKq/W7rsbRQzylxGiEm1&#xA;y2tbW9e3goQh3Izcdm5p5cQnPq6vUYxDIYg2A9E/LiTjceSE/nudY/C2U5ZkjZkfc9DoY3DCe4z/&#xA;AN89h1kWx0i+F0WW1NvL67R/bEfA8ita706ZiTrhNvQ4r4xXO3gn5u+XdJ0DW7S00uOSKCWBriRZ&#xA;Z5rgmWSVzI3Kd5GHNviah3Ylj8RJObpurzHb3OHx/QwTMp55Ru/rP1aQ2vH6wFJiDCoJG9DuvXp1&#xA;xb9PweIPE+i9/wAeSV+X9S1bUpZHnEaW8QCsArBvU/l38O/0ZAmnfdp9n4McQIfWa63t30Bb0n8q&#xA;I0l/MHTEcVRvrFQfa3kI+kHK8v0OB2fL/CxXUy+4vWfyja8f8vdJmidXVvrH7mQcRtcyj4XUVHju&#xA;G+jMfURqZD0XZ4rDEe/7yzFL2PkEmVoJGNFWSgBJ6BWFVJPgDXKXMddWFtcywSyKfWtn9SCRSVZT&#xA;0YVH7LDZl6HImILOMyAQOqwS6nGk7SwJPwatusDcXdCdwyycVVlH+XQ+2NlNRNUa96763cVg/wBC&#xA;m/ff3hrD+6/4yfvN/wDYcsbPcjhG+4+3f7ENqEst3ZahawNPZTJGwjvPSd6Gho8SoQXK0qFHXESU&#xA;w5bjdJmt55IdJJvrmSS0eSKe6+qzCf1Xg4icRvHMqP8AFT94vDi7U7DHjC+GbrbbzC7y1or6PqEs&#xA;TzGUQwS8nitp4o39W7luQoB9SOkKzBECuxNW2HTDxI4DV/pCbXPmTR7YW31mV4Wu3eO3jkhmWRjG&#xA;pdzwKcwqqKliKe+DjFWy8M3W1+8JmCCKjcHJNbx7/nIT/pQf9Hf/ADIzK03V53t/+D/O/QxPyPr+&#xA;n2cUsd5GHYD4SadM5j2j7LzZZCWM7NXY+uxYOITDHNevo7zUZZIhxiDHgM6HszTSw4Yxl9TqdTlG&#xA;TIZDkUuzYtK6KR4pFkQ0ZTUHITgJAg8ioKK1DVLm94CViVQbCvfMbS6LHhvhHNnkyzn9Rtl/5K/8&#xA;p1D/AMYJv+I5Zqfp+Ltuw/74/wBX9IeqflVFHc/lxoLMXH7gkcHdOsjdeBWuY+f65e96iEeGIHcy&#xA;C90G3untW+tXcBtZ1uAIbiVRJwBHpyVLVQ8twKV+WVMngP5tMV/MbVWHY2+3/RtFmdiFwp4ztb/G&#xA;JfD7gmmn33l0+WmaRR9Z41rTvTOD1Wm1n52gTw27XT5tKNIeIDip59cyiWZnAopOw9s7/FDhiA8y&#xA;FPLEoqwv5rN2aJiOYoae2Y2p0sMwAkOTKGSUd4mkO7tI5dzVmNScvjEAUGL0ryBJx1T8vk/nutc/&#xA;C0Q5TIbT/wA167syF4IHu4vvL23UPrP1R1to0lmfigST7FGYKxYVFQqkkjMCV1s7iFXu8T/Pv/lJ&#xA;tP8A+YIf8nZMzdN1eZ7e5w+P6HmWZTzzsVWRxRR8vTRU5sXfiAKsepNO5xZzySlVm6FfDuZl+U6m&#xA;Tz/pSFmWv1ijKaEEW0hBH+dPHKMwHCXZdl5ZHURBN8/uL0f8n9W+qfld5fuJpoUiuppbaCKQMpaW&#xA;W9lRFDrz6t/k5VrB+9P46PWxhwimJ/mP+XOutppiVbnU3e4u76DhCWS3kn9N51QrJLxSaUO9DxUV&#xA;6bZHDIBrnllCcSL4eqcfkF5b1PSdL1GSWKS0muvQdvXiIVqep8HxBG+AEbA7EnHNIEsvElLJL+aK&#xA;A+38e6m/z4nuvq2jK6GJg9wSUbkjbR/ZPwtt7qMcFXu63tczGMcBIPF09xYBoXle/wBXQvBOwAFT&#xA;uc1nafbWLSGpRdTotNqdRfDIivMpbq1jcadOYZJmLg0pU5sdDqoaiHGBs4eeefFMxlKVjzKBM0tB&#xA;8bb9dzmYIDfZE9TkqPqly7z3lkX5dTTHzxowLsQbhQRU+ByGaIETs5fZmfJLURBkSN+vkXuuh6dY&#xA;X1/d3sqMZ9N1W6e0KyOiK7wiF2ZFYI9Vdvtg0rUb5p9IDwm/58/90XruK0+bT7Q3TXaxiO8ZDEbl&#xA;AA5U9ATSjU7cgaZkcIu+rMTNV0eQ/nzHdRweX0uZlnlH1wGVU9Oo/c0qtW3p1pt7DpmXpL3t5z2h&#xA;IJhQr6v0PJVdlNVND0zLIBebQ95M8MDSKK8dzlmOIJpydLijkmInqk2m+YZ7u6MPADeg2y3w40fJ&#xA;3us7Gx4sfHbMfLmg3mv6zb6RZvHHc3PPg8xZUHpxtIalQ56J4ZizkIi3QafAcsxCPMs3/wCVDeb/&#xA;APls0/8A5GT/APVHKfzMfN2f8h5u+P2/qZF+XX5Y695e80jULy4tZYIY3jf0HkY8pF2A5RoNu+VZ&#xA;cokKDsOzezZ4JmUiOVbMh8jeRdZ0HTvLsV7qKSy6Ra3Ntc26KXjY3JiK+jJ+4ICGGv7yNmPI7gZV&#xA;klxSJ73dyO7Nsgh83fm7/wCTD1b/AKN/+oaLM/B9AeM7W/xiXw+4MSE0gjMYPwHtkzAXfV11KeTS&#xA;4YqzH8vfy9/xh+kP9P8AqP1H0f8AdPrc/W5/5cdKenlOXLwuw0Gg/McXq4eGul8782YH/nHwAVOv&#xA;0A/5dP8Ar/lX5nydj/IH9P8A2P7U80L8rZLSby9dR6u6jQpNReJ0t1V5hqEAhDrzeRUMZHIclcN3&#xA;Ays5rv8ApU7vR4PBxCF3XX42yLSdGFtqd7bzX73U0l9+lmUIyBI3gFvHFIxdwx5xmT4eI2+yAMxj&#xA;RNdzmRuMSe/ZD+bvy20PzTfQ3uoT3UUsEXootu8aqVDFqnnG5rVvHL4ZDHk63V6CGeuInbuYV5o/&#xA;J/yvpGnwXUNzfSGS9sraRWeE/u7m5jhkIpEvxBXJHvln5mXk4f8AIeHvl9n6mHxp+UbMElHmCCX6&#xA;q17JDI1hzSEWr3oZgpaoaGOtVqqkqrlSaY/mJeS/yHh75fZ+pkXk/wDL/wAieaJ79LY6pbRWqWc8&#xA;Ek09oWmhvbZbhH9NI2dKciu/wkj4WPxBX8xLyX+Q8PfL7P1M48uflJ5b0DWbfVrO5vJLm25+mkzx&#xA;Mh9RGjNQsSHo/jkZZjIU3afsrHimJxMrHu/UjfL/AOW/lnRdC07RoUluItMkWW3upn43DNHctdxr&#xA;JJAIeaJNISEI4+IOQnMyNl2kjZtlOQQoy2drK/qNGBL09Vao9P8AXWjfjiryH89WgMOlRx3RuPQm&#xA;nilj5IxifhC4RiByrwdT8ZrQg98yNPzdP21XhC/536C880HzDeaWXEMzIGHY0/XUZh9p9lY9TXEN&#xA;w6fS67JhPold9Dt9vL7Uv1G8lvLl7iZqs57/ANcz9JgjhgIRGwcfNCU5cR5nv/QeX3IQsuw5CtOl&#xA;ffMmI5teXHICII6fpLJPy5/5TjRv+Ylf1HK8/wBBcnsr/GI/H7i978kvzTXD4axer/wLAZrYx4Xq&#xA;9NK4n+tL/dFPZbuKN/TFZJv99Rirb+PZR7sRknIeLfnk+tPNpn6RjgjgEt0LD0WZnaLhbkmWuwbm&#xA;StB4V75l6bq872//AAf536HluZTzrTKrKVYVB2IxBplGRBsIKz0q3tpmkVRyPQ5bPLYpz9V2jkyw&#xA;ESdmdflXHNJ590tYZfRlPr8ZeIen+jyV+E7dMw9QPQaZdjkDUxvfn/uS+iJ21D64I4Zo/Sda+n6R&#xA;LoOhcyc+PXoOG/yrmBvfk9nYrlu1Ba6pFZmL6zbmcH4JRA4SnVuSGYszE1NeeCpd/wCPmyuF8jXv&#xA;/YrcNQ9aI+vD6IUCdPSbkzdyjepRR7FW+eO6LjXI/P8AYt4aqI5v30DyEg2/7p0VRXcP+8flt3FP&#xA;lj6luO2x/HwfOv5r+t/j7U/X4+rS358K8a/Vould82OnvgFvFdr1+ZlXl9wYllzrWsCXDCr1v8hm&#xA;vFi182kccstbP4ZZGjWn7/fkqSH6KZh6u9qej9nqud/0f0vWGF7dXfDlGNOjFJxxYvJIOqBuQART&#xA;9rY1+z45i729FtXmv+qahLbSRXF7wkdvgmtYxEVT+Wkpn3Pc/dTBRrcsuKINgfP8BExRJEgVamgA&#xA;LMSzGgoCzHcn3OEBgTa/ChI/Num6/fWMK6FcwWl/C8rx3FwivwZrSeKJk5xzAMs0iEmn2eQ3BoVW&#xA;G32h/nHp+nve22q2l/qUVpdG4m9GD6zOy6fS1gRUtYlZU1BpJEqy0U0PKtAqjfy3t/zVe6+v+atU&#xA;jutJlt3SK0eBbe5WcSKPUZFghIRgrFAxDcSvJeVTir0HFXYq7FWM67+Xuha55hg1y/aRpobObT2t&#xA;1EIjkt7hZElVn9MzglZTQpIpXfjTk/JV5R+cPkzQ/LX6PvLB5UW7At5I5XVkWO1CRw0YgOeEbhKu&#xA;x+FV9ybsMqNus7UweLARvr+gvLzqlsrOkhKPGVWRSRUFuHTff+9XMjxw6X+R8l7EV8f1Kk/OWzJj&#xA;qrsnJR70rTMjERYJcbBLwc9E7CVH5se0iPVJL4rOT6ak9qUGZRHDZL03aebCMO1X0emflwKeeNFH&#xA;/Lwv6jmvz/SXneyj/hMfj9xe4eRIzPb66PUdFGu6iGCHjyAlpStOQ+gjMPIKPwH3PV6eNRP9aX+6&#xA;LK4oYoU4RIEXrQCm/j88rb3nX5x+UfMPmL9Efoe0+tfVfrHr/vIo+Pqelx/vGSteB6ZkYJiN26bt&#xA;fSZM3DwC6vu8u95t/wAqi/MP/q0/9PFt/wBVcv8AHh3ul/knUfzftH63f8qi/MP/AKtP/Txbf9Vc&#xA;fHh3p/knUfzftH63f8qi/MP/AKtP/Txbf9VcfHh3o/knUfzftH62Rfl7+XfnXRvN9hqV9pvp2sAm&#xA;5v68BoXgdF2R2b7TDoMhlyxMaBc3s/s/NjzRlKNAX1HcfN7Xbw+kpqecjnlI9KVb5dh4DMN6ZUxV&#xA;2KuxV4B+aPlnzJe+e9TubPSry5tpPQ9OeG3lkRuNvGpoyqQaEUzOwzAiN3k+09NklnkYxkRt0PcG&#xA;K/4N84f9WLUP+kWf/mnLPEj3hwPyeb+ZL5Fr/Bnm/wD6seof9Is//NOPiR7wv5PN/Ml8i3/gzzf/&#xA;ANWPUP8ApFm/5ox8SPeF/J5v5kvkXp/5KaLrunjWYr2xubD6x9W4y3ETxfCnq8uHMDk3xD5dfY42&#xA;okDVO97Ewzhx8QMeXMV3vWY40jRUQcUUUUDsBmM75vFXYq7FXYq7FXYq7FXYq7FXYq8e/wCcjHVN&#xA;P0Us3ENLKgO43doUAqu45FqVy3Ed3XdoxuI2vc9x/hO9HnXc8Le8Z1eSO/gjQlPTZmVl4yMaGlEN&#xA;SFonxb75fxSPIh1RwYompYpk+Q93dKvly5Kpj1N5IWSdRDx/ecSCSeQYUJQihFRXbbx65Lhn3tUs&#xA;2kAMTCVj8b+q/wAdF8Fvepdh2dPQIYOgG5JCcSNhShDbVPWvssxx3udmnUajTygRGMuLp+LZf+XP&#xA;/KcaN/zEr+o4M/0Fj2T/AIxH4/cXs3kbVLLT9H8z399MILS317VDNK1aKBcEdqnMTNzHuH3B7IRp&#xA;nGVJdirsVdirsVdirsVYL+a/lLWPMtnpEGmW1ndPaXU88qajGs1sK6fcxRl4yyEkzSIFYV4NR6EL&#xA;TFWM6TafmrFqmmXWraNe3unaHfh7K2Fzpj3LWr2N7bK3L1YAXUTW4l9SRiX5Mh4niFWReTvLOu2P&#xA;mb1r22aC005daiiuWeJkuRq2qrfRNEqO7qIoo+L+oq/EfhqBXFWfYq7FXYq7FXYq7FXYq7FXYq7F&#xA;XYq7FUn8x65d6YLCCwtEvdR1S5+qWcM0xt4eSwy3DtLKI5mVRHA32Y2JNBTuFUo1H81fJmjq0etX&#xA;31W7gJjuo4YLu4jEscbyzrFIkA9ZIRE/N1X4afFxO2KoiT8y/JUc5gbUT6oYq6iC4bhxmlt3ZyIy&#xA;ERJbdw7tRV2JIDKSqhNM/NXyxc6Fp2pXjS2txfWkV41jFBc3ciCUW3wj0ImL0a+hX4V35exoqxvz&#xA;brn5V+edHsn1bUL2GFYIrhLa3glaUi+Fvwj4xw3HqSD6zBySIll5qTswyUTTVlxcdbmNd1fpBUbT&#xA;/nH38tdU0+G9tbzUJ7G/jiuIZEnQJJCyFo6D0h8BWQnj036YePyaxpiP45X/AJv/ABKZR/kF5Njj&#xA;WNLvUAiAKo9WHYAUH+6csGoIcGfY2KRMiZWfd+pKfMf5Q+W9MFhBYG9vdR1S5+qWcM11Dbw8lhlu&#xA;HaWUWszKojgb7MbEmgp3B/My8mP8h4e+X2fqQttY/lL5Q1OC/wBQ1e9g1LTZP30CxzXUHrxRPJMs&#xA;ckVmhmSERPzdacafFxO2RnmMhTdp+yseKYnEyse79TJkX8tI7PUrC4e7u7XUtUuop7w214EF1qNx&#xA;wmggvbeGNVjM6iElJPtURm5bZXKRLtCbTU/m15DEMcxvZwsqxvEv1G+5t6sixxoqehzMjl1Kx05F&#xA;TzA4fFkUImL8yPKM0kEcNxcSm6NuLVksr1klF0jyQvHIIeDRlYnJkB4rQ8iMVS0fnT+Xa6Zb6jPq&#xA;EsEFzEkyK1rcyNRoGuGAMMcqv6UaN6pRmVCKMQcVZwCGAINQdwR0pirsVdirsVdirsVdirsVdirs&#xA;VdirsVdirsVdirsVdirsVdiqQ+c/8NfoyH9P+t6X1hPqX1T619b+s8W4/VvqX+lep6fOvpb8OVfh&#xA;rirBb7/lRHrXH1/1PU9Of1PrP6Upx+pT/W/S9Tbl9X9X6x6fxc/7z97xxVG6h/ypX69d/WeP1z9I&#xA;/wC5H0frvL6x6EPP6x6P/Ht6Xperz/cV+38VcVUbL/lS3oN9T+s+n+joPR9P9LV+p/6F6X1Snxc6&#xA;/U/7j95XjXfFVumf8qL5Wn1Kn93p/wBSr+kOFOdj9U4c/h9Sv1L1P2+Pp+r8NMVeheWv0N/hzSv0&#xA;HT9C/U7f9F050+q+kvof3nx/3dPtb+OKpjiqQ+c/8NfoyH9P+t6X1hPqX1T619b+s8W4/VvqX+le&#xA;p6fOvpb8OVfhrirBb7/lRHrXH1/1PU9Of1PrP6Upx+pT/W/S9Tbl9X9X6x6fxc/7z97xxVEX/wDy&#xA;pj9I2P1z61y/TK/o3l+lvqX6V9c19Cn+if70V9Xj8HOvP4sVS+z/AOhe/wDEUXo8/wBNcbT0/U/S&#xA;leP1yP6nX1Pgp6/p+lX9jjT91TFUR5Z/5UV67/4f9X6x6ml19H9K86+hJ9Q4139P0PU58fg48vV2&#xA;xVCw/wDQu/1JOH+8P1V/q3L9J+j9W/R83r/VuXw/7yep6/pb8/7z97xxV7BF6fpJ6f8Ad8Rw+VNu&#xA;uKrsVdirsVdirsVdirsVdirsVdirsVdirsVdir//2Q==</xmpGImg:image>
               </rdf:li>
            </rdf:Alt>
         </xmp:Thumbnails>
         <xmpMM:InstanceID>uuid:0400d584-8d23-fe40-b732-9733cc85b343</xmpMM:InstanceID>
         <xmpMM:DocumentID>xmp.did:9ff58c2b-f280-4d63-867e-12c31169307f</xmpMM:DocumentID>
         <xmpMM:OriginalDocumentID>uuid:5D20892493BFDB11914A8590D31508C8</xmpMM:OriginalDocumentID>
         <xmpMM:RenditionClass>proof:pdf</xmpMM:RenditionClass>
         <xmpMM:DerivedFrom rdf:parseType="Resource">
            <stRef:instanceID>uuid:6ba4e32f-4aa8-4045-b107-f65e5aae4e6a</stRef:instanceID>
            <stRef:documentID>xmp.did:7d5cc37f-1eeb-46af-98ce-55de2f07cb2d</stRef:documentID>
            <stRef:originalDocumentID>uuid:5D20892493BFDB11914A8590D31508C8</stRef:originalDocumentID>
            <stRef:renditionClass>proof:pdf</stRef:renditionClass>
         </xmpMM:DerivedFrom>
         <xmpMM:History>
            <rdf:Seq>
               <rdf:li rdf:parseType="Resource">
                  <stEvt:action>saved</stEvt:action>
                  <stEvt:instanceID>xmp.iid:7d5cc37f-1eeb-46af-98ce-55de2f07cb2d</stEvt:instanceID>
                  <stEvt:when>2016-01-31T12:09:11+01:00</stEvt:when>
                  <stEvt:softwareAgent>Adobe Illustrator CC 2015 (Macintosh)</stEvt:softwareAgent>
                  <stEvt:changed>/</stEvt:changed>
               </rdf:li>
               <rdf:li rdf:parseType="Resource">
                  <stEvt:action>saved</stEvt:action>
                  <stEvt:instanceID>xmp.iid:9ff58c2b-f280-4d63-867e-12c31169307f</stEvt:instanceID>
                  <stEvt:when>2016-02-01T15:23:16+01:00</stEvt:when>
                  <stEvt:softwareAgent>Adobe Illustrator CC 2015 (Macintosh)</stEvt:softwareAgent>
                  <stEvt:changed>/</stEvt:changed>
               </rdf:li>
            </rdf:Seq>
         </xmpMM:History>
         <xmpMM:Manifest>
            <rdf:Seq>
               <rdf:li rdf:parseType="Resource">
                  <stMfs:linkForm>EmbedByReference</stMfs:linkForm>
                  <stMfs:reference rdf:parseType="Resource">
                     <stRef:filePath>/Users/thomas/Downloads/fig2Relu.png</stRef:filePath>
                     <stRef:documentID>0</stRef:documentID>
                     <stRef:instanceID>0</stRef:instanceID>
                  </stMfs:reference>
               </rdf:li>
               <rdf:li rdf:parseType="Resource">
                  <stMfs:linkForm>EmbedByReference</stMfs:linkForm>
                  <stMfs:reference rdf:parseType="Resource">
                     <stRef:filePath>/Users/thomas/Downloads/fig2c.png</stRef:filePath>
                     <stRef:documentID>0</stRef:documentID>
                     <stRef:instanceID>0</stRef:instanceID>
                  </stMfs:reference>
               </rdf:li>
               <rdf:li rdf:parseType="Resource">
                  <stMfs:linkForm>EmbedByReference</stMfs:linkForm>
                  <stMfs:reference rdf:parseType="Resource">
                     <stRef:filePath>/Users/thomas/Downloads/triangle.png</stRef:filePath>
                     <stRef:documentID>0</stRef:documentID>
                     <stRef:instanceID>0</stRef:instanceID>
                  </stMfs:reference>
               </rdf:li>
               <rdf:li rdf:parseType="Resource">
                  <stMfs:linkForm>EmbedByReference</stMfs:linkForm>
                  <stMfs:reference rdf:parseType="Resource">
                     <stRef:filePath>/Users/thomas/Downloads/fig2bRelu.png</stRef:filePath>
                     <stRef:documentID>0</stRef:documentID>
                     <stRef:instanceID>0</stRef:instanceID>
                  </stMfs:reference>
               </rdf:li>
               <rdf:li rdf:parseType="Resource">
                  <stMfs:linkForm>EmbedByReference</stMfs:linkForm>
                  <stMfs:reference rdf:parseType="Resource">
                     <stRef:filePath>/Users/thomas/Downloads/fig2b.png</stRef:filePath>
                     <stRef:documentID>0</stRef:documentID>
                     <stRef:instanceID>0</stRef:instanceID>
                  </stMfs:reference>
               </rdf:li>
               <rdf:li rdf:parseType="Resource">
                  <stMfs:linkForm>EmbedByReference</stMfs:linkForm>
                  <stMfs:reference rdf:parseType="Resource">
                     <stRef:filePath>/Users/thomas/Downloads/fig2b.png</stRef:filePath>
                     <stRef:documentID>0</stRef:documentID>
                     <stRef:instanceID>0</stRef:instanceID>
                  </stMfs:reference>
               </rdf:li>
               <rdf:li rdf:parseType="Resource">
                  <stMfs:linkForm>EmbedByReference</stMfs:linkForm>
                  <stMfs:reference rdf:parseType="Resource">
                     <stRef:filePath>/Users/thomas/Downloads/fig2.png</stRef:filePath>
                     <stRef:documentID>0</stRef:documentID>
                     <stRef:instanceID>0</stRef:instanceID>
                  </stMfs:reference>
               </rdf:li>
               <rdf:li rdf:parseType="Resource">
                  <stMfs:linkForm>EmbedByReference</stMfs:linkForm>
                  <stMfs:reference rdf:parseType="Resource">
                     <stRef:filePath>/Users/thomas/Downloads/fig1.png</stRef:filePath>
                     <stRef:documentID>0</stRef:documentID>
                     <stRef:instanceID>0</stRef:instanceID>
                  </stMfs:reference>
               </rdf:li>
            </rdf:Seq>
         </xmpMM:Manifest>
         <xmpMM:Ingredients>
            <rdf:Bag>
               <rdf:li rdf:parseType="Resource">
                  <stRef:filePath>/Users/thomas/Downloads/fig2Relu.png</stRef:filePath>
                  <stRef:documentID>0</stRef:documentID>
                  <stRef:instanceID>0</stRef:instanceID>
               </rdf:li>
               <rdf:li rdf:parseType="Resource">
                  <stRef:filePath>/Users/thomas/Downloads/fig2c.png</stRef:filePath>
                  <stRef:documentID>0</stRef:documentID>
                  <stRef:instanceID>0</stRef:instanceID>
               </rdf:li>
               <rdf:li rdf:parseType="Resource">
                  <stRef:filePath>/Users/thomas/Downloads/triangle.png</stRef:filePath>
                  <stRef:documentID>0</stRef:documentID>
                  <stRef:instanceID>0</stRef:instanceID>
               </rdf:li>
               <rdf:li rdf:parseType="Resource">
                  <stRef:filePath>/Users/thomas/Downloads/fig2bRelu.png</stRef:filePath>
                  <stRef:documentID>0</stRef:documentID>
                  <stRef:instanceID>0</stRef:instanceID>
               </rdf:li>
               <rdf:li rdf:parseType="Resource">
                  <stRef:filePath>/Users/thomas/Downloads/fig2b.png</stRef:filePath>
                  <stRef:documentID>0</stRef:documentID>
                  <stRef:instanceID>0</stRef:instanceID>
               </rdf:li>
               <rdf:li rdf:parseType="Resource">
                  <stRef:filePath>/Users/thomas/Downloads/fig2b.png</stRef:filePath>
                  <stRef:documentID>0</stRef:documentID>
                  <stRef:instanceID>0</stRef:instanceID>
               </rdf:li>
               <rdf:li rdf:parseType="Resource">
                  <stRef:filePath>/Users/thomas/Downloads/fig2.png</stRef:filePath>
                  <stRef:documentID>0</stRef:documentID>
                  <stRef:instanceID>0</stRef:instanceID>
               </rdf:li>
               <rdf:li rdf:parseType="Resource">
                  <stRef:filePath>/Users/thomas/Downloads/fig1.png</stRef:filePath>
                  <stRef:documentID>0</stRef:documentID>
                  <stRef:instanceID>0</stRef:instanceID>
               </rdf:li>
            </rdf:Bag>
         </xmpMM:Ingredients>
         <illustrator:StartupProfile>Print</illustrator:StartupProfile>
         <xmpTPg:HasVisibleOverprint>False</xmpTPg:HasVisibleOverprint>
         <xmpTPg:HasVisibleTransparency>True</xmpTPg:HasVisibleTransparency>
         <xmpTPg:NPages>1</xmpTPg:NPages>
         <xmpTPg:MaxPageSize rdf:parseType="Resource">
            <stDim:w>98.997868</stDim:w>
            <stDim:h>35.897922</stDim:h>
            <stDim:unit>Millimeters</stDim:unit>
         </xmpTPg:MaxPageSize>
         <xmpTPg:Fonts>
            <rdf:Bag>
               <rdf:li rdf:parseType="Resource">
                  <stFnt:fontName>LMRoman10-Regular</stFnt:fontName>
                  <stFnt:fontFamily>Latin Modern Roman</stFnt:fontFamily>
                  <stFnt:fontFace>10 Regular</stFnt:fontFace>
                  <stFnt:fontType>Open Type</stFnt:fontType>
                  <stFnt:versionString>Version 1.106;PS 1.106;hotconv 1.0.49;makeotf.lib2.0.14853</stFnt:versionString>
                  <stFnt:composite>False</stFnt:composite>
                  <stFnt:fontFileName>lmroman10-regular.otf</stFnt:fontFileName>
               </rdf:li>
               <rdf:li rdf:parseType="Resource">
                  <stFnt:fontName>LMRoman10-Italic</stFnt:fontName>
                  <stFnt:fontFamily>Latin Modern Roman</stFnt:fontFamily>
                  <stFnt:fontFace>10 Italic</stFnt:fontFace>
                  <stFnt:fontType>Open Type</stFnt:fontType>
                  <stFnt:versionString>Version 1.106;PS 1.106;hotconv 1.0.49;makeotf.lib2.0.14853</stFnt:versionString>
                  <stFnt:composite>False</stFnt:composite>
                  <stFnt:fontFileName>lmroman10-italic.otf</stFnt:fontFileName>
               </rdf:li>
               <rdf:li rdf:parseType="Resource">
                  <stFnt:fontName>LMRoman10-Bold</stFnt:fontName>
                  <stFnt:fontFamily>Latin Modern Roman</stFnt:fontFamily>
                  <stFnt:fontFace>10 Bold</stFnt:fontFace>
                  <stFnt:fontType>Open Type</stFnt:fontType>
                  <stFnt:versionString>Version 1.106;PS 1.106;hotconv 1.0.49;makeotf.lib2.0.14853</stFnt:versionString>
                  <stFnt:composite>False</stFnt:composite>
                  <stFnt:fontFileName>lmroman10-bold.otf</stFnt:fontFileName>
               </rdf:li>
               <rdf:li rdf:parseType="Resource">
                  <stFnt:fontName>LMSans10-Regular</stFnt:fontName>
                  <stFnt:fontFamily>Latin Modern Sans</stFnt:fontFamily>
                  <stFnt:fontFace>10 Regular</stFnt:fontFace>
                  <stFnt:fontType>Open Type</stFnt:fontType>
                  <stFnt:versionString>Version 1.106;PS 1.106;hotconv 1.0.49;makeotf.lib2.0.14853</stFnt:versionString>
                  <stFnt:composite>False</stFnt:composite>
                  <stFnt:fontFileName>lmsans10-regular.otf</stFnt:fontFileName>
               </rdf:li>
            </rdf:Bag>
         </xmpTPg:Fonts>
         <xmpTPg:PlateNames>
            <rdf:Seq>
               <rdf:li>Cyan</rdf:li>
               <rdf:li>Magenta</rdf:li>
               <rdf:li>Yellow</rdf:li>
               <rdf:li>Black</rdf:li>
            </rdf:Seq>
         </xmpTPg:PlateNames>
         <xmpTPg:SwatchGroups>
            <rdf:Seq>
               <rdf:li rdf:parseType="Resource">
                  <xmpG:groupName>Groupe de nuances par défaut</xmpG:groupName>
                  <xmpG:groupType>0</xmpG:groupType>
                  <xmpG:Colorants>
                     <rdf:Seq>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>Blanc</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>0.000000</xmpG:magenta>
                           <xmpG:yellow>0.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>Noir</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>0.000000</xmpG:magenta>
                           <xmpG:yellow>0.000000</xmpG:yellow>
                           <xmpG:black>100.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>Rouge CMJN</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>100.000000</xmpG:magenta>
                           <xmpG:yellow>100.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>Jaune CMJN</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>0.000000</xmpG:magenta>
                           <xmpG:yellow>100.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>Vert CMJN</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>100.000000</xmpG:cyan>
                           <xmpG:magenta>0.000000</xmpG:magenta>
                           <xmpG:yellow>100.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>Cyan CMJN</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>100.000000</xmpG:cyan>
                           <xmpG:magenta>0.000000</xmpG:magenta>
                           <xmpG:yellow>0.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>Bleu CMJN</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>100.000000</xmpG:cyan>
                           <xmpG:magenta>100.000000</xmpG:magenta>
                           <xmpG:yellow>0.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>Magenta CMJN</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>100.000000</xmpG:magenta>
                           <xmpG:yellow>0.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=15 M=100 J=90 N=10</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>15.000000</xmpG:cyan>
                           <xmpG:magenta>100.000000</xmpG:magenta>
                           <xmpG:yellow>90.000000</xmpG:yellow>
                           <xmpG:black>10.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=0 M=90 J=85 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>90.000000</xmpG:magenta>
                           <xmpG:yellow>85.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=0 M=80 J=95 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>80.000000</xmpG:magenta>
                           <xmpG:yellow>95.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=0 M=50 J=100 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>50.000000</xmpG:magenta>
                           <xmpG:yellow>100.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=0 M=35 J=85 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>35.000000</xmpG:magenta>
                           <xmpG:yellow>85.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=5 M=0 J=90 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>5.000000</xmpG:cyan>
                           <xmpG:magenta>0.000000</xmpG:magenta>
                           <xmpG:yellow>90.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=20 M=0 J=100 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>20.000000</xmpG:cyan>
                           <xmpG:magenta>0.000000</xmpG:magenta>
                           <xmpG:yellow>100.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=50 M=0 J=100 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>50.000000</xmpG:cyan>
                           <xmpG:magenta>0.000000</xmpG:magenta>
                           <xmpG:yellow>100.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=75 M=0 J=100 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>75.000000</xmpG:cyan>
                           <xmpG:magenta>0.000000</xmpG:magenta>
                           <xmpG:yellow>100.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=85 M=10 J=100 N=10</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>85.000000</xmpG:cyan>
                           <xmpG:magenta>10.000000</xmpG:magenta>
                           <xmpG:yellow>100.000000</xmpG:yellow>
                           <xmpG:black>10.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=90 M=30 J=95 N=30</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>90.000000</xmpG:cyan>
                           <xmpG:magenta>30.000000</xmpG:magenta>
                           <xmpG:yellow>95.000000</xmpG:yellow>
                           <xmpG:black>30.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=75 M=0 J=75 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>75.000000</xmpG:cyan>
                           <xmpG:magenta>0.000000</xmpG:magenta>
                           <xmpG:yellow>75.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=80 M=10 J=45 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>80.000000</xmpG:cyan>
                           <xmpG:magenta>10.000000</xmpG:magenta>
                           <xmpG:yellow>45.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=70 M=15 J=0 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>70.000000</xmpG:cyan>
                           <xmpG:magenta>15.000000</xmpG:magenta>
                           <xmpG:yellow>0.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=85 M=50 J=0 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>85.000000</xmpG:cyan>
                           <xmpG:magenta>50.000000</xmpG:magenta>
                           <xmpG:yellow>0.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=100 M=95 J=5 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>100.000000</xmpG:cyan>
                           <xmpG:magenta>95.000000</xmpG:magenta>
                           <xmpG:yellow>5.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=100 M=100 J=25 N=25</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>100.000000</xmpG:cyan>
                           <xmpG:magenta>100.000000</xmpG:magenta>
                           <xmpG:yellow>25.000000</xmpG:yellow>
                           <xmpG:black>25.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=75 M=100 J=0 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>75.000000</xmpG:cyan>
                           <xmpG:magenta>100.000000</xmpG:magenta>
                           <xmpG:yellow>0.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=50 M=100 J=0 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>50.000000</xmpG:cyan>
                           <xmpG:magenta>100.000000</xmpG:magenta>
                           <xmpG:yellow>0.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=35 M=100 J=35 N=10</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>35.000000</xmpG:cyan>
                           <xmpG:magenta>100.000000</xmpG:magenta>
                           <xmpG:yellow>35.000000</xmpG:yellow>
                           <xmpG:black>10.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=10 M=100 J=50 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>10.000000</xmpG:cyan>
                           <xmpG:magenta>100.000000</xmpG:magenta>
                           <xmpG:yellow>50.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=0 M=95 J=20 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>95.000000</xmpG:magenta>
                           <xmpG:yellow>20.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=25 M=25 J=40 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>25.000000</xmpG:cyan>
                           <xmpG:magenta>25.000000</xmpG:magenta>
                           <xmpG:yellow>40.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=40 M=45 J=50 N=5</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>40.000000</xmpG:cyan>
                           <xmpG:magenta>45.000000</xmpG:magenta>
                           <xmpG:yellow>50.000000</xmpG:yellow>
                           <xmpG:black>5.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=50 M=50 J=60 N=25</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>50.000000</xmpG:cyan>
                           <xmpG:magenta>50.000000</xmpG:magenta>
                           <xmpG:yellow>60.000000</xmpG:yellow>
                           <xmpG:black>25.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=55 M=60 J=65 N=40</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>55.000000</xmpG:cyan>
                           <xmpG:magenta>60.000000</xmpG:magenta>
                           <xmpG:yellow>65.000000</xmpG:yellow>
                           <xmpG:black>40.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=25 M=40 J=65 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>25.000000</xmpG:cyan>
                           <xmpG:magenta>40.000000</xmpG:magenta>
                           <xmpG:yellow>65.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=30 M=50 J=75 N=10</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>30.000000</xmpG:cyan>
                           <xmpG:magenta>50.000000</xmpG:magenta>
                           <xmpG:yellow>75.000000</xmpG:yellow>
                           <xmpG:black>10.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=35 M=60 J=80 N=25</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>35.000000</xmpG:cyan>
                           <xmpG:magenta>60.000000</xmpG:magenta>
                           <xmpG:yellow>80.000000</xmpG:yellow>
                           <xmpG:black>25.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=40 M=65 J=90 N=35</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>40.000000</xmpG:cyan>
                           <xmpG:magenta>65.000000</xmpG:magenta>
                           <xmpG:yellow>90.000000</xmpG:yellow>
                           <xmpG:black>35.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=40 M=70 J=100 N=50</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>40.000000</xmpG:cyan>
                           <xmpG:magenta>70.000000</xmpG:magenta>
                           <xmpG:yellow>100.000000</xmpG:yellow>
                           <xmpG:black>50.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=50 M=70 J=80 N=70</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>50.000000</xmpG:cyan>
                           <xmpG:magenta>70.000000</xmpG:magenta>
                           <xmpG:yellow>80.000000</xmpG:yellow>
                           <xmpG:black>70.000000</xmpG:black>
                        </rdf:li>
                     </rdf:Seq>
                  </xmpG:Colorants>
               </rdf:li>
               <rdf:li rdf:parseType="Resource">
                  <xmpG:groupName>Gris</xmpG:groupName>
                  <xmpG:groupType>1</xmpG:groupType>
                  <xmpG:Colorants>
                     <rdf:Seq>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=0 M=0 J=0 N=100</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>0.000000</xmpG:magenta>
                           <xmpG:yellow>0.000000</xmpG:yellow>
                           <xmpG:black>100.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=0 M=0 J=0 N=90</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>0.000000</xmpG:magenta>
                           <xmpG:yellow>0.000000</xmpG:yellow>
                           <xmpG:black>89.999400</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=0 M=0 J=0 N=80</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>0.000000</xmpG:magenta>
                           <xmpG:yellow>0.000000</xmpG:yellow>
                           <xmpG:black>79.998800</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=0 M=0 J=0 N=70</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>0.000000</xmpG:magenta>
                           <xmpG:yellow>0.000000</xmpG:yellow>
                           <xmpG:black>69.999700</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=0 M=0 J=0 N=60</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>0.000000</xmpG:magenta>
                           <xmpG:yellow>0.000000</xmpG:yellow>
                           <xmpG:black>59.999100</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=0 M=0 J=0 N=50</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>0.000000</xmpG:magenta>
                           <xmpG:yellow>0.000000</xmpG:yellow>
                           <xmpG:black>50.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=0 M=0 J=0 N=40</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>0.000000</xmpG:magenta>
                           <xmpG:yellow>0.000000</xmpG:yellow>
                           <xmpG:black>39.999400</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=0 M=0 J=0 N=30</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>0.000000</xmpG:magenta>
                           <xmpG:yellow>0.000000</xmpG:yellow>
                           <xmpG:black>29.998800</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=0 M=0 J=0 N=20</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>0.000000</xmpG:magenta>
                           <xmpG:yellow>0.000000</xmpG:yellow>
                           <xmpG:black>19.999700</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=0 M=0 J=0 N=10</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>0.000000</xmpG:magenta>
                           <xmpG:yellow>0.000000</xmpG:yellow>
                           <xmpG:black>9.999100</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=0 M=0 J=0 N=5</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>0.000000</xmpG:magenta>
                           <xmpG:yellow>0.000000</xmpG:yellow>
                           <xmpG:black>4.998800</xmpG:black>
                        </rdf:li>
                     </rdf:Seq>
                  </xmpG:Colorants>
               </rdf:li>
               <rdf:li rdf:parseType="Resource">
                  <xmpG:groupName>Couleurs vives</xmpG:groupName>
                  <xmpG:groupType>1</xmpG:groupType>
                  <xmpG:Colorants>
                     <rdf:Seq>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=0 M=100 J=100 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>100.000000</xmpG:magenta>
                           <xmpG:yellow>100.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=0 M=75 J=100 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>75.000000</xmpG:magenta>
                           <xmpG:yellow>100.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=0 M=10 J=95 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>0.000000</xmpG:cyan>
                           <xmpG:magenta>10.000000</xmpG:magenta>
                           <xmpG:yellow>95.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=85 M=10 J=100 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>85.000000</xmpG:cyan>
                           <xmpG:magenta>10.000000</xmpG:magenta>
                           <xmpG:yellow>100.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=100 M=90 J=0 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>100.000000</xmpG:cyan>
                           <xmpG:magenta>90.000000</xmpG:magenta>
                           <xmpG:yellow>0.000000</xmpG:yellow>
                           <xmpG:black>0.000000</xmpG:black>
                        </rdf:li>
                        <rdf:li rdf:parseType="Resource">
                           <xmpG:swatchName>C=60 M=90 J=0 N=0</xmpG:swatchName>
                           <xmpG:mode>CMYK</xmpG:mode>
                           <xmpG:type>PROCESS</xmpG:type>
                           <xmpG:cyan>60.000000</xmpG:cyan>
                           <xmpG:magenta>90.000000</xmpG:magenta>
                           <xmpG:yellow>0.003100</xmpG:yellow>
                           <xmpG:black>0.003100</xmpG:black>
                        </rdf:li>
                     </rdf:Seq>
                  </xmpG:Colorants>
               </rdf:li>
            </rdf:Seq>
         </xmpTPg:SwatchGroups>
         <pdf:Producer>Adobe PDF library 10.01</pdf:Producer>
      </rdf:Description>
   </rdf:RDF>
</x:xmpmeta>
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                           
<?xpacket end="w"?>
endstream
endobj
3 0 obj
<</Count 1/Kids[5 0 R]/Type/Pages>>
endobj
5 0 obj
<</ArtBox[0.712845 0.0 278.507 99.4425]/BleedBox[0.0 0.0 280.624 101.758]/Contents 46 0 R/Group 47 0 R/MediaBox[0.0 0.0 280.624 101.758]/Parent 3 0 R/Resources<</ColorSpace<</CS0 48 0 R>>/ExtGState<</GS0 49 0 R/GS1 50 0 R/GS2 51 0 R>>/Font<</T1_0 52 0 R/T1_1 53 0 R/T1_2 54 0 R/T1_3 55 0 R>>/ProcSet[/PDF/Text/ImageC/ImageI]/Properties<</MC0 56 0 R>>/XObject<</Fm0 57 0 R/Fm1 58 0 R/Im0 59 0 R/Im1 60 0 R/Im2 61 0 R/Im3 61 0 R/Im4 62 0 R/Im5 63 0 R/Im6 64 0 R>>>>/TrimBox[0.0 0.0 280.624 101.758]/Type/Page>>
endobj
46 0 obj
<</Filter/FlateDecode/Length 1633>>stream
H‰¬WÛn7}߯à£`iÎðþØØi6A'FA' d9qcYŽ/mú÷=Crµ+Ëv¦0,iə!çrÎ̼œÿ½¼T¯zzt¨º/Õ–"²^Ûè•sÚyV6i¬º\v¿©sÈ<cÔÇ«®lSH"•Á_£ÀÐ+ÞQ3äƒIj±ê^¬Œ:Zw¯ñ÷¥‹VgãUÒÑ´£HlXëî=*fŽ'˜‰8¹Xq9»X,¹DÛY´s–÷ÚÙô¿VMqæÐNãá4S´HýÜíÔ_jc×m=\Í:¥¤z˜5¬ê'îð¦#c´iNÚä zÒOõ³Íbv"Hz[-ÆbY_uÑh¥žIÇÌêº¯'jí Vœ!gý¨Ø«4`8¸Ð›9ëìœÄÀÝy»§³ëŸ»ƒý.¿f'](‹AÖɇ¢ÏˆålÕíõû³?Š(Uѽ¯²ŠBR!ÉI´¥¡
Þ6	Åg¶e?
²í"=	Ná‹QγãnïÉ a«ªµØ"ïèá.Š%D"e±øn‹ýÙ[_^/÷?Ì~'Ï0I5;êö×ç®Ïn®O×çbzkïÕüâª,"»ª:'.—x{u3?"Ù"Ǹ?¶$Ev;RÆöN{b;•½+¶¨@|M"ûlTAÀ }BQ	òP8"7t0Mk>oÅ&jŸ¢œhŒ+gb1¿^žÏ‰‰÷ƒ/FG⬼ÓÆßbök»ªºÝÆQÒɅ!°#NÈ8^EMv@×#¶NGG`J|)ŒtQ¿}C0i"ù´@©|a‡Õ¢ÃOæTt	7èlÄðŽXP‹í(
ˆMª¿cÂ¢;Ù¦xi}ˆ*9MÜd"y)VB*vhÄ1܄Ÿ ò)m9A°åü$÷ŽTnÀ‹¬mE¡¤¯¸Ð)P?p½:"‹Åœë£Å:3%(œˆÚ4ñD'?g"—
1"û9Ò)"˜`ªr¶­œý˜Üíp/ÎÉ%`¯(ð¤8ÐpåçónÐÀP†Ø?Jíµ`ÃkßH	½E°«ÈB†¥~©E(T,@èË1ˆ+Á1-ë·$I#I!®,3
YÁÕFˆ¬ŽH&¬:Ãw™Û\`Ïìl	y€WHÙÒqcÇ­Ë6 ZÖ°Ä~UGsFŠ
€Ä¸–676öÿ8&ì3Ê`šv¿ÇóQÛIƒpsÆh£ð¹{0säÍIQ债ˆZ¯dð®7&ilï¨vM¬]'»>´Vè<"°DÁj±Ý6êz­(Uj®Z›bönÖ§ÁE`-0l¶6"8ýº|ùö[♏ø."ÉäeÔìåÁãðÙξÕç¼Õì}V 5—ZŠ>}ùRI²!<ŒéI@Ú{'ˆ÷ª|~0êxZŒm0ͨü0%ƒë•ò1Óâx‡Xï0XóøÈq§'‰¶Q¶e¸Dðz‡qȔ6'и{P£û-:W&у#È_Y0…Ì$x4Øncÿð¸è<iÆ1ÃB@A£ëôÓ#…AIÖ)Èe-]§bR$ƒñÔÉ`Ëé CÚ</@-Í)nÃT'S	áqÒÃpil"r¼4B‹rxŽâw°be8Eã&8eU,µ Â`%ó»Â!¥ÕÖ§E'³TØ<{"v,=ö\jÅ,m·°`°öHz¡—y˜<µ:ÿT§çÉ뀌ïn—æjp‹²ŸÍÛM´÷(«´KGТÌ¡ÈKרV§Û
ì0îTÛÏXA,1"¶Xöb…,è lÊDSÔSU¬;ŒPGˆ)Ðx4º43Œ×±bT"•÷(™mRðÞ[\ì=HðýþvR
[Fˆ[É£"Ná0él_–1.r‰"Arªé³Eƪ
Ÿ‡W6ÿ]}dÓÉQ©"åƒ
á¡KJKÂk¥M¦8Š©'sº]øŽ!eÓ´pG÷ïë6ƒ}žRô@"õ€*°`³­/F?ìË[Ñññ©ÌÞó3uz~².K—«2Ž«"ËõJ­o.Õj7(4AH/ÏÚÔðÖP—ßò-w˜Ó[)ç7×R(EŒÐR'ÉÖÙæt5ÿ¸lUóìÕ¡êþ`íQnä
endstream
endobj
47 0 obj
<</CS/DeviceCMYK/I false/K false/S/Transparency>>
endobj
57 0 obj
<</BBox[56.723 47.762 65.9259 39.9716]/Group 65 0 R/Length 69/Matrix[1.0 0.0 0.0 1.0 0.0 0.0]/Resources<</ColorSpace<</CS0 66 0 R>>/ExtGState<</GS0 49 0 R>>/ProcSet[/PDF/ImageC/ImageI]/XObject<</Im0 67 0 R>>>>/Subtype/Form>>stream
q
/GS0 gs
9.2029335 0 0 7.7903902 56.7230167 39.9715784 cm
/Im0 Do
Q

endstream
endobj
58 0 obj
<</BBox[93.6735 55.8476 107.767 49.5476]/Group 68 0 R/Length 50/Matrix[1.0 0.0 0.0 1.0 0.0 0.0]/Resources<</ExtGState<</GS0 49 0 R>>>>/Subtype/Form>>stream
0 0 0 0 k
/GS0 gs
107.767 49.548 -14.094 6.3 re
f

endstream
endobj
59 0 obj
<</BitsPerComponent 8/ColorSpace 48 0 R/Decode[0.0 255.0]/Filter/FlateDecode/Height 134/Intent/RelativeColorimetric/Length 730/Name/X/SMask 69 0 R/Subtype/Image/Type/XObject/Width 155>>stream
H‰ìÔE"AEaÜap—ÁÝÝrpwhœÆÝÝÝõ7³8'¹`šîÌêzÉ
bκnÄ/ªªZí¨hî_ç!¿H'öƒißH'ö•i_H'ö™iŸH'ö'iH'öŽioI'ö†i¯I'öŠi/I'ö'iÏI'öŒiOI'ö"iH'öi¨1ígýh÷)âj¹dviw)æ]Ë$´;Ô­TY Ý¦¨/43íEѾg'ÚMŠ¢ýílF´G«m+Yhש	ZÙ²@»F'´Z63ÚUŠ¥½·—ÚŠ¥µ?›í2EÓ6˜ËíEÓþ<›!í"ÅӜµ,Ð.PAš…,ÐÎSÍ墝£Úc[Y ¥šËD;CI´-¦²@;MI4—‡vŠÒhÎRh'©ÍJh'('ærЎS*ÍÙÉí)ҎR2Í09BŠ´Ã¤H;DŠ´ƒ¤HÛGŠ´½¤HÛCŠ´]¤HÛIŠ´¤HÛNŠ´m¤HÛJŠ´M¤HÛHŠ´õ¤H[GŠ´µT2­R¿8Új*ûjueâh«(+­ÁÖCVRéïZqY ­ Òikš§-§ò¿Ð²@[F?¦iK(­ñÐC'­¶mq<m!Yк;Z - Z­³ÅÌ<d.™ÐjØRhs(-jå!³É†ÖΖD›Eyhq#™AF4W@hÓȊ暠M¥´Ø‰‡L&3š+Nk¥´è…‡L ;š·ML¦'{ZüÀCƑ!Í%ÊmYÒ\AÚh²¦¥<î!£È"æ*SŠÐF'1-éiN¶´´<d)҆"m)Ò'"­…iýI'֏i}I'Ö•i]H'Ö‡i½I'Ö™iH'Ö‹i=I'ÖƒiÝI'6€iƒI'6"i#H'6–i"H'6i3I'6ióI'¶"im¤HÛLŠ´Ý¤HÛOŠ´
U;úû-À©ÿ 
endstream
endobj
60 0 obj
<</BitsPerComponent 8/ColorSpace/DeviceCMYK/DecodeParms<</BitsPerComponent 4/Colors 4/Columns 155>>/Filter/FlateDecode/Height 134/Intent/RelativeColorimetric/Length 8736/Name/X/SMask 70 0 R/Subtype/Image/Type/XObject/Width 155>>stream
H‰ì—{lU…Ç—^"áƒáŒ9'B&ʐ-ÅÄ17¢²9¦qº1&‹¤ãýèʄ®<RÊ£Ð,­0
´…>€>ØÀÀÔ‰ÙÌBԈ‹±û~çwnÍ¡¹½½¯–þñÕËé}œsÏç~~ßßáü=w¤#éÈuÓc_ì|Ýä¾Ù]â–D_k˜	‡'.©
â—Ö:x‹6k7Ä/¬%	s‰¾¾(²öÕN
◈Y‹çュ܋öv=²Ö;Ð ~‰‰×®'ÎÚûõEÀÚ7¥AüÒ1CãÀR;b.FîW~é`­ƒµh³6\ù¥ƒµ$à0Ñ×eÖF€+¿´˜µh}¯mô»Ž)sm€Áp¹\ù%î¬%éw˜T¼%úZZÉÚwÁ•_"bíZß­çœêÇÌqrÏÜT'ó:׏NKeê¾óò
š'ó5µw-֍X¬¾8"ÚaKœý£'˂µƒW4fÐÊÍÀ5NÜ3îsøï{¸ï‹">Ÿ­ç`ç:?Ä=çÐuØuE…µ$`'¬W~‰U_qæ²å2årԔc¦fÀڔš;ÖuªéŸÞéÔíNúmœ¼mcàd߬À‰>HïMê^[Õ·2فªžÛ¤ªgŽð±Ãßø>—¯9Ù7Óy}¿õ¾_M"ŸÏ
1b³'I=W—A—;þfŒ¹¸²ÖÜo¼%ïÕJç†ÃÈp嗨°æs­^ÎBŒ¹÷'÷tà*‡+—)ò&ÈGu¯ÍÊªì±]*oÙ!Ýs¥¢[žïš/å©û¤<X ¥)…r4𺕿9ÁãҔ")ÃßÊSäXç½ú¾¶ò¦]ú^|O‡ÇÍÊ£²Ӎ¿U®ùÛ0æ\Ç%Ú/qI"¬MW~‰U_S¯'5:!ä²eê/—1z†÷¹'¯ì€².*ºï6®
ÀŽÃÔaðtXÊ!)Áà_eR,åR$ǤáÿyŒ;ˆg–à™Gä
)
ë{Ïc]òÁߞ{®î2Õ}ê=—9sÎÚ끵(xm¸òKÌvºÍËý`œÑ!Œ™¿nÞ¥ÇYEÊ	y9¨"•*Kû¥Rþ*'$Ojd§üCvÈÙ.g-gp쟲Gêõ9¯I•2Xlüú{êG—;g72§žÃœuüÖè6eͯ¯µµÄp†NW~‰åÊß¿v5—5ÎMÜ?ºC9Ó9™£÷ZæaŒ\Àd¤·¾ª•!²"#oÊyK2å=Ù(ïË«òå"Ž]Íò¶dËy启ÉWî*•Õ`–ìæ#0rç¬zÎxÃo~¹ý^kN‹2k?W~ikîy6sê6/kœðg¦úœñ^Ó3ì\%ÆX£—òå"ú+Þrøº rIVËe©|,Kä3Y,ÿ³\űOd%þ–Žçl{›å厌æIì3ב¹¿ãÓԘè}Úí0·]ÞØãÔmœ¥`Mg(÷ƒD8Ío/ˆ³ÏZÂÚÓàÊ/±ôZÈmÜAC¬a~öuœ¦ݽÜ8s]Fö™Ç8·È¿¾ÄùšsŸƒÌBfZfÙ±4"쭐"9ºœ'×\›¯ûå¸v;~&y#ët+gyÝÆ–ݍ¬¡g֍X¤ó3áŠ5ÃQ`í|ÿ~‰5kŒî¢ì;ìk구ï§ë4ÎMv~—3²—eË9õÒzÌÇÕò¡2–f\M·óçïåIÿ
™fϙkÌ­"+Ê)g®ë¸|ã
íMyãîÁ="³"¾uYÓÊÝ R§µÆAñæ.J¬ýß»_âÁšº
^à,Ò¾†ê²Æ~î:­œqn:>;kœ]ԙÈùHgýÞxš'<nûÍ#–#!O ¿D~‡ÌF tyËRÞΙߪuV³¿q«¥_9G]Ö8Cu7Àï¤Ý9-BÞÂad¾o¿ÄƒµÛàÎ$öîêk:Ãx¿áúf‡ÎÍ·"3Î̅ò¹r6ÝüEž&" 㐱–qvìac<þÆf+y[âí]e™ýÍuw…2kt/¬NCH8±d+Ê^û¾k¿Ä‹µÓ˜?º#ÀœMÕ½š²vD÷MÞz‡ón­\ÆÜüT9{ÎÃÙãj42
áÉhãn'¹nŠÍTúí0»³˜;g)ç4=ÊÞV'3(:3"»÷PvµÖ:­éý¼–C¼ÇãÉZœ.ks¬77MÜXóº
¾8Ñ{"d]÷³»À«àZà™›.gdi$2€|ËÂǃáȽÈýæ·'Íá/!Ë°»f ÿћ;ÐÛ¸ƒ‡X+òOçêüäþÙZ§5õF¼y
çwЂ"ÃHšígMOÖê]·
\"ÂÎVÙc»îGŒµ}`m'\³YÞÆü¼¤N›k½rŠÍÆÈÔíHß@ƒô±|½Sƒô3æøœ1Æ&{ݳȺ+\U_nÒ9zF;Yãe_#ÿü°WòwÁ®5w$cb0CÙyüO֔7̣ڡ˂ôýQÑm"Šµ¯5²öŽ¤ƒ5Ìi"ãmF'32E¾z¦4È-–ÁùZ'‡?>ç.›µ?Dž2?ғì€ÁŒfg£×8CÉû±Î{á´lŸœõ;-'ï&˜‹kKäñK¼YÓY
·±éÅÌ*M)TÖ^C_#kìîépÏBùBž·øˆÇiÌgäìFðõ•T'|Læzœ™z§Íۇ͋ÜK_F¸×f*kg"oîä½¢[ž°GÖôÇüdO‹Ôi-á+'œÅh†.—+â—D°VϼÎê¶~U=st?8Ú¸²¯9^»¬šaœL´6̜F'+2ÖÕâòFùœÁæÁ'ŸØN:ÏX£×¸ïbj*çÚÕnÞ¥ûgíÀU)ì–qñYs[8Œ¬–ÿˆ_ÁšºmÄ¢ ;=r¼k¾îERŽ=´F{»—µ'<¬ÝéaÍuZWO\ÖÜ9z-ÖØ×vb7("cØéü¬ê¹Mt'@O‹·/ƝׯQbmv/¿$ŠµÓØè6v#ú¤,Xˆv^Š®~B¶bå®èî ®×ƚ×89'ý¼v"u¶~¶§ÞkûyfûÐjùPyÞ
‡º]­¢{®îÚÓá´dò\+Y[/Å/	cÍë6ìôŠÓÙª$Gޔ?ƒ5î3=}mœõ}o_»©I_ã±>Ö׆ùô5ò»Î̖ó'/§ð™G"sÎrÎtö´¤à,VÜyßËïq¼¶A.ˆ_ɯM݆ŽÄÁ£œm™8·¥Ø]怍©ÈdäóÔs™¢Ãȗs»Ú(Û]"ü!·‹å*~c—t/ ×% 3\6pM
»dBgg¬ý֔©ž{8Œd¡oû%¡¬Ñm#çßà¸-;@¿Ð3»¥NgÜjô*μéž9ú}cÈåí‡/¦¯ùlí«®Ó&[W{Y!ÉFpœ‹}·]íhàuÝ	´§Eâ´x¸-–³2¬mAòK¢YcØÅ鶊nypÛAõÍv9ÿ| KäS™Fž1f~`³t´ÍHúëÛ6WÙ±QÆ{ÚcÈÓ洅ò…ü	Ncd/äÌæìæ~R;xE°Ý;­9Ö¼†pÉFòK2°Æ.N·UöØ.¥)ERß°·gÉ{²=žn{ޘyÜ\5ÞæéÝÈHË(;6Î8›d]=í%d¹|¬NہùY(ÇaÐ7§¡§±;&gñ୅×#9ø~ýÖ"¸œ_'ú8n+'C²_*Õmdc9æ^ší¤Sm§œdÌ=ˆÜoì±Ï=d{Ädcó9"o)8ˀӶɹÓÊSB»gR2æš{Ÿ(ym'<ᗨ°æw¾-¼œ_no£ÛH©äIî‹œ¥tRšÍÂ_#O!?µ9Éò¨1ös›¹3ÌgKä3åŒp®™=­4P,ÜGØӒÚiÑf.Ü×·'µ\Ü7¿Äl†Fpê†/rž'²PŒ4ON¡_—
rQVÊyE>WOÍ´áYsÝTãkšùo6²Àæf†u4î…àŒ»'ýI²+^ŒEéšÂa߬ø%úZ(cætfGgW?Þ5_g)DÑoå}ô·ë¾°ÀœE¦fY^°y™f.[…=v=¥ÏÈwŽCx×ò`Tߺ5@ÖNKm3N‹5ka\S8ŒìÅ÷엤bí>Ûúgè,eŸ"oìñœ§ìZYò.ø¹¤;EîËÕP–á£Ë2ÑõÈ(9cÿcG+gº`v²#ÆÚm'·f®1F
¤Bü1kÍ}ç͝s÷ªvè²àÉÛ6ê,-*#.oÜè)îìqéÊÝeM:òöËȪºŽãvÙ÷½7,«q6Þ°¼A^A¤Œ`ƒJ‰
æ#3ª¡˜Ôř"ÔrCkT4ÉL3b	eÙÝË]ûžšœÆ¦±iš:ý>¿sþ—ãåì½÷.6Ìw8sö¾Ïç|¾¿ßOå}ûl QÙĉøl·lôrUp›½ˆ?™»dæ"ÎZ'^Û!³Wf-ߍ^c7"	ÝdWxGǬÅù'xêaŽ¦¶š5ψó~)çžÆ^
Ôé¬÷º0j8£—égºóؤûú¥|]³ÁZªÜuöÜî'k;e¯óJVYëâwÔ=a]jÏn°'߸?¶	Gǔ§­zåŽà¼å.ƒÉ7ÎövþX(Ãg^°{àͬsÒ[Üwü0ò¶\'¯äŒ×â~Ïöa6`Äðö{ù÷V`Ÿúj»tãouÇ9¢á™ÍvÊc`s¯<zÁöÀÁK¶Ø¢ÝÉLxÁµKäš~ÒXs}g?Œ¼#¿¼Wr†5ïV=ñüêá›óÞ¿lKXÁM{û¼©û¾Ú)J¯ÂÁcxïmñ5û¦Í™ìÒÃô±v§ø²§ï"¬Ç|¦î>ggëâ9~yW®€Wr'µ.~3؀å­ÿ‹¶ßòÞc½¥ŽÃ]pgçzc3ã©Ï"3f4Ý;éNñeÖYè­~óÉڞÀ›¯$µ‡vÆJüq| {'ôžÎnŒámþï´SaÎLÌe¸ŒÝ*g2ï±Ó²kxî^ß¡»ï–ídš1Wü0²WÚÅ+9áµnØ;6áÁ|Xav;ô¹gµO«'Û"'˜Ûç"c\VUúJàà§ÎsvtèOòbݙȵÌ6S9ȟFöåox%§Xë$5Ó6V}(f`¿±/à­ªÒߨçŒU_Ö=@9"]€þ¥;ñcÆ>s®r–.ý0²¿àՀWzk"ÝfoÌúºÔaNzU£Œ=§î;<àé>G˟èKÿ²cdåsçgiŠF"¾ðJÚYK×÷÷øMéA؁!åMö¸ÂañڜÉ.0üÑ<|ˆ{C9ș_Öª"+¯ä"׺ùméAåMf7ºñðÀŸé<FWÚyºçÔgp6æá||˜u&.Îü²v°?]sazkê6í҇c¼á/vTãÏÎèΚrÇCo¾X»äù€WrŠ5?¼	;0¤,1‹	WÌp¤zøæ<TŸÉîªû@¶y¸ˆ8ó˚Î5É9Ö|0¨]*,Åxƒ/Â1œIÏjwúa÷ÿIˆ]_¬ÉÌì•^ɚ¸
–"7™ý•9"ÇÊÙ¤ûú¿˜»3ìô"×_þT¯ä,kÝü–5Ó¾_ ³›ô©òE"=8Kº;ç|÷|*×kæ~»øø¼oٙÿÍó¹j]	©]ðsÍÝ¥&u‹î²síe±\wÇÇRëþ›óx÷kx½‡yùLæsò™Íçw§40é‹5v6dœ5óýÒpßÖLÛhûMøÒÈ1œé>ègr3f¸r³d¸j
/KnÖ-½-X·|M°~ÅÍÁúVëWÞŒ|í«¡zIdÕÊPä–C'Õׇ#·­Ðœ¸cyøÄ]ËÂѵK5sÎü]ËsÏçµä5yí:yºå·ÚïIx>‡Ã¨›Ëƒnö:ãÍ}Mº¹6~9RþD_¯ä¬×ü¸M˜ÒÙ
ÞÎêÎø÷rqvc†­x®âxŠ±´nI8zÏâpôÞëÂ
ß[nØ°0ÜðƒkÂ'ï¿:|êG_zh¾9æÜÉ.°#®ÿŠý\^CxŒÄ³hŒñ·&Æ]­áÎÍß©;Ö|Æ#G‡lî땜fÍ/oÒ§ä¸ñY2óŒq×ÅøOp픱[•¯ˆñ•aËáªÁÅÜÀÐéMóBg~<7|æñ9¡Æ'g‡>3xö™ée瞟ZªÙ:EÿçÜÙ_Ì6>5+ÈcyÏ5Âhå="A|høÎëî¸ÔwÜo1¿ÁZæ@?ŒT4Ï+9͚ß.…·T8s¿Ÿ‹5õ™‹3íÅ8ÆpPŒ/ñÔéGæ…Ïl®¶àçܯ¦•ÁTÓ¶ÉeM¯M(mÞ1¶¤ygEqó.ùßDÎñ·¦W&•žûõäÒ³òœF{¼&¯ãÎxÏ0ç¸ÏjÇÊgæá^‰y-
NóÍÚèMy^Éi֒a'YÎL¸ÿM‡â4<AgÎèÈ»—ÚÝct¢p þ2|á,a¦éՉÊVËnakϨâ–#‹Úª‡¶Ö-h«r>r®íýa…-ï,j~wt1,*{Â'œâ=åNVîÄwnæà^oô*JŸ֘×ÒÀ™oÖÆ>˜ï•œgÍÉréîÿ8Ö´;™Éð™pÖàâÌxLû‡ÁþÂ]ÂMËþQÅ­G¶N~¡ ã젂ö–mƒ
‰sîtyA{}¹r"-¦¾ÆëãJ"9º×	ÏÆs1Þį±>5n3¬¹ûÓïo"*kÈ÷J¬ù¹^©zª'ãç3ʵ‰u¨aÍqšv—ÌN†³Fã2zÒñ˜2&¼¨¿"6_mmÂÓ;>Æ>XØþÏAvä¸ãrîorîÏWt4Éã¢åÊfëÁEÍsðÇt2þÄ£Æo°¯n"ÏhXÓe^3NKÓïcS7öóJÎ{-M÷cB¬ñ8f6vÐxÖpš\_íÍÇlŸáf-˜ÀG­Ò‡°¢®o)cðôŸÁEí֐âvk¨dx‰Ž‡ó7"9õ]ã`õNÔnÝeÏtðÖhü&ûs¢º}UÜf³&jvƒ4Íi‰°V3]v5ä4kÉtd:Xs»MºÈ°¦û€\W®¯v'N£7¥ãÔg†3Çeq<¦Œ
-nµF•µXáfkܧÏYã?Kš¬	—¶Xcû·Z£C°×ñßò"åò¯.ÇÑ«û¿‰;aƍÛð,ÝcMîíOv'4÷'/֜]->ïЮú´3ž²Á•Y§Ž™M:Iç5¼æ°Æuf^×îd>Û=ƞýÅg:I¶;œµZ#Jaì¬5ñóÖ䧭©ƒNYS$SË9>cM¹¼Ñšt™Í܈RõŽƒUá­Íñ›î
´/0'âWXS¯Ñ¡ìÌjñNË`‡ÖÌþN'W'öZ:™óÓ¡]1Ú¬¹Vê¶%·Û{¨xƒ±F²ÈüNÏé|&ó{‡Ìûp&Ž'<c°Õ`͵fVœ°f7á\ƒ5m˜0w®ÃÊ~ƒ7éSV·Ñ¥Ò×øôÌãs"µ¼Æ¼&÷ƒéÏæ´L²Vyo±WrºC»ë՞f0·‰Ûè&Xkp±¦;ýɾ(0_©Ó>pféD\g'­+‡D­닓k­Ù3I5{6ÿ×[³¦ØÌMo°	£:ñ3ÈÌG/·I?ãOÓ£†5\{BœËýÀ}¡Në¡nðňôWRf-~‹ÿ-â"4üFI³fÜæôhtÝÝ
kºˆkØ™­t®ÿûàÂvuÚè݈³NX3Ç	[Óá«ÆúÒüj«rÉqkÎ\˜‹X³&Âl¨Ìx%ì©ÚǧÏ÷èÇXcþuV£?ÝNËkµ֖x%ã^K3™b0·Éoè~ Ån@‡ÆXc' ?áB6´?á©kæÜS°uÔª¼ö°5w	áXÎ-"?X"Iº–ÙNg·‹ÛØė­ì²Àšvèc•ö*üGV­éNàå´4Æk‹î,õJV:Ôëº{1áõ˜TyMòó²×Õ¯¸9hf6º‹Ý ‰…5qsóUû¿ì9
^à_á-gËYóVŽaÞpkܦ»©ø'NfG`Œ±&»¼ãXvuštýñÊõÞsZ&½¶øëe^IŠµd¯Y"¾óËd&Xs»Íéѓ÷_¦ÃØ
˜×𚲆ƒ´?G•™þ"8''¸'±ƒÖü‰á
ñncW`7ew¥G™Ù"5ñšv(»ô·™Õà¿S§eµº¥«Ë¼'0k=ÁYw¿E:û7…ÏƵĺ#lX¨3s{(ó¬µÇXÄM8Ê՟°¶ÌpfbX3=ê°vE<kmÕönß8Þµ?Ù	˜ÓŒÓºú®™`Mf[¯dœµD®ywË0k\Kö<u›Ó£tYÓkJÙC™×zÌkÌkìÒ׺ȬïìŸuË׏_µ®Ä×÷Ìkô¹G'b­«¾ë	>ҙ½«;©ÌmѵKÃÌ屙M樶ˆ³ôļ&Îl90²‡6JžÞ4/½gqîuNKäþíaÖêų^Iy7HôúõrÖÔmÌm«¯3+á<Ó²»¢¸½¾¼ £MvЏ¦onu߈–´¼'¬É^Ðøäìý‰ÓØW.pZ–½¹å†WRòZ*Ì¥šl±FäÚÖ¯¼Iݦ=*žiÞ1¶"yŠ®ëøÐôèè̜´®µfVÀî'+˜#à Þ;aÍoœö?öË-Dª:ŽãOÍîìììPO'íê¶æ¥MÍ̼äºZˆl˜¨˜ZI¥]Ä®F>=AЅ
*è%ˆ "Šè!*ˆ @Âܛ»º·ÙuFzIQ¢âôûüfÎ4äÇ33ç2sæ<|Ù³³3gçœùÌ÷2cu_­ùyA؝¹!–èŒÁóÔÇ·%؟º	öíýÏÓj‰µGw¥Lr-C+ᤘÑ⟦ó׊¯åߋímºdâ73?ærT}è'0b-h™ÜFXՅgáop…àŽŸ<fs†⇶§'ŸÙ±y¹®&ùI?ÔM œÓÓLžVêZý`íàŽ"IUg¨_~äƒnù*ÞFo"ˆ·Ù9ªÞ&›Q;Ö?Íá
vØ	d#<áq°…8fà}0™¶–ÎaWd­ÎøÙóEž&}^×êiÒÓ¶J"}>°Æ=1©b_û¿?_‹—Ùg:¿×¬ÍÂ5ù5|`—z›nÙ£t*ݬÀŦ$OáiÌZÙwˆc¼ñÀgt>Ùzšl2Oƒë"âÚÓ¤;–}M~°öÜ֔I®dh9Ÿgµ¬U{^7½¸÷p|h÷>ímì©Wµ's°¡Y*;áì9a毎fºÁ>—¶–]‹8Î1¶$ɞ çeÿèh"‡3§æç²ó›î–©OV$Æ_ëMéӞv™§ÕkòMªÖܒ[š×`ßÁyäÝ6lÞð7ÍӋ¹L…9˜"[QV%Æ.åØÔ-kw´£‹5;ñÍS/mÖí9¸í±dOÞÓʽN?XŸ7©"Ö\þ¼\Q@¬'c|ö0@gŸxçÎ6<húë›ãʛt-¶i&"ëpY:ØÅüv¸"?ÆÇÎå2"®£pFÿKvkbâý5I²ÿÚû`²¿Ô¸ÒõúÀÚ¨|'L

kNï¥ÿs`ó"-00ò̽©Ó/ßÕx'ú›lÓ3'nŒe¥wÁœæªäc±"Cö"x™îaÔ挎F>Û{`pëã­U}§|`{`'ï;4"¬!~ä¾Ô¨t`Ø(ð&ž½pæXWáYô°³*ø'ÃìP.3aOL¾\9ӎ&ù£Ù¹ý@²ÓÓ¥³³X"ë7)t¬]é~ºqNÓß%×؆ö.{ucjòƒÕIò4-{aú»%q8ÊÀÜñ®&¼NÅ1½Ƥ›Áٔ0ÊÎcCì~àþ6ü³ê®P)gù×;adìõž¤I¡cÍ_sx.v'f©°1úâå
c/àSÚá$g¾_ÇëдázٗË°9!ŒŽ¿)œIÿ#—ٝšë_¨Ž³jX+Ã×Æß^—4ɓZêºg{Ž‡ùVõù^«ä;,yj[
O*ðöÑÊ~sês'­¶`ŒnÆsðBüŒ~C㓃;÷']ñ4Ÿ|mü½5­&…Î×¼âÔ¡t'¥ð&žTàMö)~5)وÏá_Á˜t³‰w×&égêgláŸØr(QÕ÷»Z֊^ï"®Ó¤Ð²æV†–{ɹÁ{žh…ú<Þ¤¼I7k}<Mæï½òÅ1ŒÉß`ÒæìäÁ©!éhødÿÆgã%ߟGߛŠY"ï"I¡d­Ò3ó9y¾ìú¬Ø¼ÑßÈEeN¼‹>¦'¼"±Ó¯lÊí€<gÃíicwjvºyUp攵Iñm"BÉZ©{[-«½
Fw>œ¤×ÃyÊ>…'˜ƒ-•ãe°8"Lêæ"üÚ½/ÉÖèï=<»§¹ý=tpmN™úty¤гæÕgs¥×mx>®YJwÂßØøÖȑ>åΖ>&,ªŸÙœ±;ek8z_n³VâõŽXûbi‹Ik~>+õ6²TØ)ð&¾¥G®âc0vH¼Lþ¦œIÏ££ivŠ?úv½Ÿëˆµ¯ni1©¡XsrO«è2—I¼Myv"7ÉS¶%Ì
KƒE匎Æî,µ"FÒß.‰›zÖfã£ZïrÊä ½†
¼	WxXAò˜r¶sr@r—mQñŽ©֎.l6)ô¬yÁU9Ìñ»4ÏÛ ô7¸–Š"1yLýL8ó=;=èkÓ?,l6©!X+¾¯^ñWê˖"!X"OÙ§Êâ¥×)g¥ö@
È	#3?-h2©aX+ş×þÆïÒ¿´»áo•2‡8ÆÏèhp旧yÉÚ±®&"†µ ò³X0$YZà
¾ð99VÎèh²%¿On°v¼3fRĚœÙ'¥<oÅRÎ؝NÏSã¬e†æÅLjÖÜà¯Úÿ‡·Álå™+pVãÙYk#–A¡g͏ì,‡C›7ºâ¸²³,ÖÆÚ¯2)"¬ùÅW%~ÇóaÉ>՟uå°–Mύ™±oø›­ ï—Û¬e"-ƒBɚŸ¼¹ñނ¾W.³–ùmn̤вæ'{Õ¼Ÿ ï‹¬ý~}̤P³VËÞf¿¿ ï'¬eÏKf:ւèjuȌ§¬]ho2)t¬Å[Ð×\C¬eþlo2)t¬E|ÏÚßó›M
kAq× ì9bÍꌛ:ւêk
œ3Ö´˜*Ö"¾j'µ3ÖM	"BŚ›ìýÞkTN™¶·™T׬•
È­FÒV÷5&Õ5kõÀ[Ð÷'Ö¦¬¥sLªkւæ¨ysÂȄµâ:""Ö"ÖÜfmÌZÙnRÝ°4/ŽY;eÝÞiRͳ4
ÌU¥¬X«™Tó¬Õ3‡Aߟ€X;i­í6©.Yš¡ˆµ'¶Ö­0)b-âÌmÖ­uw˜T—¬Õo!dÏ	#'¬õ=&ÕkAóñ戵_­ž»Mª+Öꍻ ïQ@¬ýbõö™TkA†5ÍÚ1kãv"jÆׂæ,âÙ5Ö~¶6í1©\Ö"EŠ)R¤H¥õ¯1¦3^
endstream
endobj
61 0 obj
<</BitsPerComponent 8/ColorSpace/DeviceCMYK/DecodeParms<</BitsPerComponent 4/Colors 4/Columns 155>>/Filter/FlateDecode/Height 134/Intent/RelativeColorimetric/Length 8872/Name/X/SMask 71 0 R/Subtype/Image/Type/XObject/Width 155>>stream
H‰ì—{lWÆ"Ö^¯wGUÕ
jb»¶q8‰Ûyرã4ʃ'È¥iIÚ¦Ò4&Jˆ* E)ªREU¥'¨(¥P©*E¢¨ª Ò(±w×ë÷z½»jÕªJUU<.ç;3w<»¹qg׳;þã"G3÷5žß~ß9¯ÿ×´ -è&Е¶ï•Ü4Z¼4o*ô»:"FJ=BSiµÞÜf-ð¡©´ÀZ'0Wè÷s'µ[?-4•²f-Ÿ¿÷¹ò-æÛûdÉÚç>%4•râk7góýý²`m'&4•24,Í#æœ0RM\©´ÀÚkn³¶"¸RÉ5ÖòùM曊€!7Yk$®TʘµB—bgaž3脑âJ¥œ±ÖqlZG½¬®#Þ+Ýß5ÔsxZ_>Tõm|ôzm:è"êßrÀÐÖo—[Ú¶?Uögæxûª=äþ,y&yNœYžßþN7bcž2–	k­Ä•JY±¦úŸÚ×vÆ$Wv–$7ÄCŸäeû·üý;ö÷ïzÐìÝë~}?¸ûþÐý÷B{vzàÞ@è¡{ôÐý¬ðþ]zøÀN}à',\ãž|Îc1Â|ZkòÚ´öâ=±·UɧEɟ»yÌÔlXë"®Trµ^"×iœ¥0fgk×¾T®$O'ÉÒ¡íúÀw¾ª<¶MߢGNlÖ#oÒx·>ôã/†Nö¢kÜüÁFcÅž‹5ˆÇE;ƒt†~æoŸÅ~×1'yË7kŸä›™¬39aänâJ%WXKWémø.¦Ÿ±YŒ=hðϲ±%¹ŠH¦Àq††OuFžìÒGÎtFžnŒ>ÛêûùÚòñZ|ã/6¢kÜÃ3Œá±4s%‡X"׃´WŠÒY'';éy83|.µyäU™p鄑­Ä•J®Õkéç´³&ýLr&=ÌÌCÎ@xÏѯ°±_'O
?Ñ­<ÕÉl=·Î?þüšrfêå¦òè+¾‰×–•Mü©Á;qŽþJÑ=<ÃKs0—Ù£µ°&Öfîh/ìÉ{ÃódîÒÙpFæÎ,ýÍbm&O+49à+SÖ¾F\©"3Ö üþMÖ¸.#Ÿ€gXœ'Ÿp¶Ùcÿ:mð5
¾È«¢`ë÷+™­Øùo썻Jc½«4~©¶dòr'ÞW=-º¿P[Âch¬dk`-¬9úL›{`/éu̝ÅÊXð3½Íbm&O›K¬å0C{‰+•rÊ~ÿ²^k¨Ïàifn†î0j0ú֜"ð1Ê=ÎGò£¨ô/xן—x'Þ¬÷N^¬ñ$'UžøàžäX…'[ìIÆ+J ¾Æ½á*cq‡9<—ÖHa9K{±ÏÑޒ7œÉÊSö¶}kÈPôÒÓnô½
ÍPŽ¹sÂÈnâJ¥Y±&Ï9Ó{p½fgMzeüÌâLzeû˜É<Œý+dòõÎ"OâýÅ%‰«ÄØý½VahʸÇϒw˜ƒ¹XÃbŽÖÆ¨í°§Å2•Î"g"¬q†'µ®#ÞOüF¹b!}¿<ûY&¬=@\©"S_"ÞFÙý2ÔdûÓÓ87©–Kçì/äc"‡ÈFx{q¾'ÿ­,MˆjoBԐ¾Xf×Õ^<c1ž7ZÉù
OĚ)¼¡–ƒ¿!O©á¾µ›d
JgçütÒ{Ú£fË°¬}"¸R)ç¬AäìmTgs½&Y£ÌÂ÷…¯ †âÚììªiÎ.N{Yò]Óǘ±廊/‰e·Lˆå·Ž‹·C¸Æ½I±Ô1<sh®åq´&j9æöâ<¥½qÔnVŽJÖРVƒ§9ù7úžÅ.Y{"¸R)/¬á9zähï^®×,Öèû¢NGý4þR"ë337Qs¥pö¿ªÒIQçOcbågGEÓ†EKŐh©'p{xf0WçÜäGÓ¼qG^Éyúêò2ìÉÞFg@Žr_C½F¿+?Uï9×}-ޜ0r˜¸R)/¬A¨ÛȐI܇¢^"¬Q~rFu;ü¾ƒ‹k|ª»ìœÁ»À؊ˆuõ¢µ!,ÚVj]Ž{ƒbu5ÆDEãm˜" ¹\ǡΣ5¹~3½
{rÝöÔ4k\¯Ñ¹V³{š"Ü)4/ٰ岯%®TÊk$ÎQêé¸f£^µ'd
ߛóóܲ2ËÓ¢Fð1±Bõ˜ä,"ÖÔˆu
AÑÖÜ'Ú[¡~Ñގ¿¸g0·¦vD4߁9Ì­'ü€¼ÖŒÓÚÜ+Ð^ØS²ÆJg
ÓïÀÊO»§eãkéßóFsí÷óÉZžæ"µĕJùdMz[9Jõz>ÔkÈ/f
=}ô‰ʺ8±öae	êýI±$0*V}ÁÈ­µWDG×e±¡ç'èÜá÷ÀÆ`,æÄDƒÎ=e)֌ÓÚØcâüRÓ&kt&üpFî	è̳fm&æŠÁ×2F¾O\©"WÖ ô¤äÈ(ÔE'›õ''»tÔLÌ}î	ï4ê´k"}¦§¡‹ˆÖ¥'3ðõ¶èÜúOѵÂ5îáYP¬_|Åd)÷©ð6¬‰EOJ5›Å!òø&£VC~ª<͉fòŽbT2ôGÚ4•òÎZDZRøz"°Y³
Ÿêæހ3"X‹_ª-IŽVzïQ}õ1ê´úrÔûð©h[‰¼´q¶ó¢»µä
c0VzÖà¾kÒÚ؃}
Jœã'ã[Œü¤ž ÅÓ2ñ…,ý¢(˜s‰µ"Ú¿4•òΚÝÛÌEM>òt{ ŠÞJžÃ¬Q­fô2?×օÄú&ÓÓ6KÎÞ=÷B&o;ðÌð¶¶fÌA‡5£\ÿÑÚØ#v¾Á‹=GŸióãªÕp&ô/8£ãZ,[Ö
í{9ÊПhW5•
çº
=ùˆ¬ÙÆ_lö¡7T³†ž`mø±³&9"'Þ&st&ÖÀ5ö9ÓÀŸÜÀӜ棛šÞ愑ÓÚ{šJa
ê9ì…ÀG]È°ñçהG_]Î}(굜ùڰه¾F¬Ñž\«ÑÐ(=-"oãƒùä+ƒ3;a䌖ÔT*k$ém‡¶ëèeÍ{³ÞQoàB½6(VWÛë5^"úPì}¥Ñ‡='Ÿ8Cèþû8"ã÷qÛ׊ÅçfÉÚOµ"¦R!Y»ÒuÄËuùÉù
²lü¥&úÃD°Ê"x‡¸˜ZœUŠ1Ó}èŠÛ¹EO›\ìÁÚ܃R­†=ÑZžFgrün¹f-ÜÙ×R]»àkÏj1M¥'²oÛøhü¾"s5÷¢Ñ
Oò*ñFÙ's>m+ÀRŸhßpYlè_®qÏ¢u¹ìAc¢Açüü°'×ä"ö¡Å‡=џ¤xZ±±æ¶gÙϞá»8aägÚ¨¦R¡Y»Òq¬"ë6òÔçè	'mÈ8d]ò]ò5ÊQémF°¦,¡#¶Z'—®q,b̈h^"9"¢Î‡5¬ü¤ZMæ'öSžÖyôzO›éýæ"k3yœK¬ýBÒT*8k¦·¡n‹<¶M~¢[Go;OýèeêGámP@µ˜'¼
‰–ªˆXWœ[®qÏ0Fr†þk$b‹=Xksÿ‰ž€ödO£3düns™³tÖ¾F~©…5•
ÂZú\xÛ¶ýåðö6ô¦·q¯(I^­0{Ò:_L,»½|õ؂pM÷îÀ3Œ±8ûˆæÒé=úö4ªq†Y¿Ç\ä-ÃwsÂȯ´ ¦R^Y›éÿÙsØË=)ÕNìmf݆¼ã,5yKü»'ò´Æ‹¾u¼+*oƒp{x†1‹9ñxgçä[u¥VF{ÀÓ°gŠ§#kn27KŸvÂȯµËšJ®°æÒo	ކº
}¡Õ"ž[V¿P[C&Þ§<22•x*Sqªå î5é{Ƙ¹	ΰg'­™Ò{ҞYß|³æÆÿ{–¾à"'ßhok*C½f©ëˆ·×>øÀNù†>AòÆþ$#JÌ¡¯LS‰k†¦Ì{xFcxlÐô3Z#zv•krvÒÁÞ½~ì™õ÷KŒ¹äÓN9«]ÐT**ÖH}›úB{v¥C'{¨«Æ_n*—¼¡¶Ìq®RŸš"Ü£~câ}ÕÜsb.Ö{nkr?@{ôo9à›Õ7žo¬9x''ŒüAû»¦R±±Æ}ÕꡇîÑ#Ç·èçº`$
ÞP¿½A¼]¬aŽ«ñAêF+Y‰á*ã=ÃŒÅøÖàÖäìD?Ðy4{O+kùâm†wtÂȵ¿i*eÍZúy²=¿ÊÛ¨VG¾!ç"ÿg¿\€«ºÊ(üß$BH"Ñ¡­´LÒÁJ)•Â@©V¢"*/h+´ˆ´""¢´ (È£¼)Ãû
4)-)"H
"¦¥>ê8NÇюÅqĵþ³ÏÉár'œ›{îÍ;™59wß}öyìï®õÿ3ϪY8 Ëæíý×ïkyåp×4ö"`W~wszŠÇ»'ï8çJr"~¶¾w+®ÁM³sø˜ëûOYóý|~ɓbñRĬÅÊ£Ãæ0ߪGÊ¼ðÌЬ‹³Óޔ¼½·¥gúûûz¤Ó¯®äwKû à^õ:Ž9¦^†9¬õ˜ÁäŒk\˜ü,®Y5xbýý€ß½m
֢宮sëZ¯¬"ñR°®SÒª†>©YÊڍ¬­ß6=Îú‹<©ÏÁ¿ÔÃp¬cÈLÎq8C/À54;±&×¾©Y‹§·…=§FÊñR²ÙYJFlÞèo5/÷ͼL#sð9ú—ŠÇÓÌÄÎå9Ú`ˆ³óSÖnxV?Œ¼-ù⥸²é»Cíμc0,ë³߲xC¿P³´_æå•}2˜«dK…cŽñ;ÎQ?Ã9¬Ñ4;‡Lh¥ý€ß{
ðww½îßï¼zÎñÃÈa¸˜—š"5?ç|mrKöŒçÀJ5x£G±Æ¿ôâ£ê[ÌȚÅý3U8æØ¥y39‡œñœê1#3¹†zZ¤¼$2kMàm~)7ÄKêC#ñ€hß[¿Ÿ·¨üæ¤ôªaã2ªÇŽÈÔޔ¼¡?¥o'9²¥Â1Çø稟áæ0×àZA¿ûÿÆ\òÃH!ºN/%D†6ôþ™ªYZÅÚ
ìЫØSÒ·.Ld±e¤cìègè+xN%ûN¬Ñà}Ý,¬5!~9š²W¼sւx‡[}'f)ê{2Äúíü¤¡Ê•úÄcŽÙœù£';c½a÷›œÀ¥FŠS÷ˆ—bÊZï5½f©Íj0ö–d®ÚH1¦¹‰9UCŸ´²Óo?+þ³€ä‡''ôâ¥ÀX‹Çû8%­jÐÓédÈፙ
s"1õ3Ìaîòœ[Ž¯&âÌ/kÇÁ•—'µºÞ%k{ö¥¬ÝÈj1rUÍRÆ0fs¦ÙÞē…[Œ3¿¬h½Y¼"¬Õ÷¼¦¥'¡J›7ô§ÊÅcæ¦Í™W?ÐԌÜä¼ùbí¶M⥄d­¾wÊÏÈEíÈې	­XéxlsÆìôڏ¦æã&æÌ/keí²C^JXÖê{fÖúÈRå
õ›ú¹ã19Ãwuö	º‡qQÏ틵öëC^J8Öü¾7on)gÈÙ¸ý&nBoŠF~9ù…•!/5kÑ>7k~Öc.ޔ3Ž…÷
ÝgתxhÆ
:¦Šg¦ÖjVóÔë…Tßò:ßµþ
×öº¿¦d­ÓŠ—Î×"áÐ捵ÕguÝ·‹)‡³ïgzÎn¦ºÿ—ÍÊ¿<'åL—RÎÜ7WUÞ}^Jy·_»´ ¥üÞߦ"ß³0YÕe±êô]K'Ow^š¤ºs¹êÔíµ²Çô{΅¬sYëpMŠë»¯‡ë;÷Â{Ã=ªÌ=×r‹ç©Aû¸ÿ×!?ŒœºsY'—ŠµHg<‡YJ17ù¿¡u¯ç:®pqfóe³åì¯Í8pâ»$7V#+քNv\z§Ä:¥Ý†PY[jc¨´Ífôc[äDÖvÕñŒÖñg¶ë8¿ç<óx>×9Ùq­µ.¼Ábs™Ã¥òèæÐðç°ç0gñí¾ùaätçÅI^J(ÖÃçÓËlù™ï¾F8k†3Ý+7c6_ƛ4°ÿSࣴÍ&‡%rT'–#ǚ¿&Å)ûåhJ®…H¼)‡%:ä¨@ÞÒñ¢ä<Wœº_Ï;ž¾ÛâÑ°hsè0høSö®ãÎåy6oqdMïÃC	ÅZcjˆHןv.3G=
~feäåL=ŒþEï'ÏÔò¯j½Õa‹œÔrõ–²"/Gä É9&¹R"û¤TöJ™Q©¼.'0~´żByۜEþ
Co`½ýXw¯®<c‡^\Ûܩ﹙ãïÂð¦¿ÃZ{狵®ó"½"P¬EË[¬rO"5ÛÓÎàeÆÇÆà7ôzù*¤Êb«Pò¤•(S»å"ìJÙ"çd£ü^6ÈEè'þ߄Ï[1¾C*tžÅ_	Ø´Ø;"?]ÑpgyÞ.½¾2ǼÅ}ñw@Þ´Ö³ýÍf­¾~!hÖºówz£n	Ö¼ü*
_Ô¥¯Ù¬!7énÎè/êcØ{2p"'1$¡zyÙ-§•¯ÍR­\­"+²Jþ,ËåCY&qÄÏ«äOøþ=·E¹«"pGÌSÏ+R¿³™ãuy}æµÅ[¶ú›Ösô6Ã3"ÏÑ;ˆ–5ðí¥ˆY«kOƒb-ނ`Íö6öÌ ›5zòJk2ì/÷™S¨õ×!ãc6cgd›TÁ¿.ÊzðC¾ÈÔoä2W>'_É5™
½`þϑÿÈ<ù—,"0ïCY
î²¥FýŽëìv˜+6>—¯×ux£¿ÙyÊ,Åý*k¬Ùàigëó´°væYͼ"p¾oÖꐓ£.Öè¬Ñ™_ÜgÖd6gô²=ÈJæ }ìUyWÖÈ
cÿTžžWÏA?…&»4ՌςæÊ¿ÁÜßåe0·V>À:–Ïíº{Ç±'SÞèo¨é±ü
\ÇêLÞƒžÖ*z£ñP`¬ÅÒs'äÙç{¦·©÷ÃjYÛb]N/)JÎÕڟûN¿±8«T/b®€—ѧèc3
O¡qÐ(h"ÑHh´šf˜›'We±üMVbzùÝ©¼•¡Ž+Ö¼fbÓ[Y3jŸÊ%kÌP;?ò´X°†kz)°
"¿êzî&`Íö6­ÙPk;¾†¼:Ö"G=…ÞÂÞqúȝÈMò-—ÎæÈe†ñ®ñ†­ïBƒ¡Ç]}Ï0ø"ñ½êqŸÈï°Î*"©ìX²o`ýv×/Jγr¬Ñ×X¯•wY"Ìüôåi±`­ïs-¼Ôh_‹WÖEÂG¬Qø-Ú9ª½ö'¾F֘Ÿ¬ÕmOc]ż#‹ÀNjÈÌéàe'ñ­¡†«P¨·KC@ƒ aÐXÃçLÃÛä0ó˜õß6x'³ô²"ý)™'kìWxڇ‹}{Z,Xëÿ³4/%t†6"«±f
²½{È>"þÁ½emÎcÆ~q<íô™¬íYç?oxù±ñ²¯ÆzA= /A]¡îæ3ÇûB߀¾ox›jò"õ{Uzk·=òŽÖmnÖÊÚnDºÎÉOߞÖÎœ'楨YÂßÂs2üù£õ²(X³½{Èe
Îúˆ¾F֘gì;7¢NcÿÈÌcŸù¬ÉÃa†³¯¦îî€:¹t—áî+†Gúß Ÿ˜žÉÚm-XÞ,çµ/Í5¬1CÙ«"¡=Õiuˆ|¦ÇK)úýÄZåcÏ´ôRÜ}-(fâŚímÈ%ÖBÜÓã;u™¡dµÚäÛ
°F²=m"©ÍúA÷ÎÈV‡Ð5ùlR­:âóí.Þ˜n4š
±7]ƒ¾"LÛ¬VÖråDÖv"Ÿ¨Õ"õ´X°6hbº—š$C½ö݋	¯9Ñòژ÷Œy¶·i͆þ€ý÷:×øÚÔjËÑ̗µN{Êåi½Gä¬=¸º-åšdA™æ›d‹?ú]7è!sÞÓ»'Ýù`˜µ k6²–§¬åK1NÏeÃ:-–¿_¬}û©V^jk^{´ßùe2¬¹¼ÍÎÑâÔýHЃºçÜ{›µyrUsï	ãMLv2'é_䊌µJ­U¦áíó!ËûÈæ@Ã*™ý…²ö±ÃZê5öGP3kþš"ÂkmO;ë·ˆ!kUCÇ·òRĬł³†ž;Èüâ=³:ÝyiRY»ìk6öoÊQÝ{2@ÖØ7N3µý`Sï³þÿ¢ÉÎÖÉ_i.e4³Æ?—d1Éíoz×ñÐtk¬×Ø÷""í˜çìYÊ»,jœ§Å'µaã2¼wÖêÚóºæôŽ'`­âÁYÍmo³r4)V {±÷d`¹ö W=Y»#ÖX¯±ßÝ'¥Ú—Øù©=Ac=-¬
"á¥F±V_Þł åýhÝocn1¿Ø²?Ø*çÔwȄ݃1ÌØÚ!,CÓÂ2´£ÉОa:bÏñ
úÐmR¥}ÁÐV'–£ý'ëHf| YkçFÊôRÔ½A¤>w"³¦ÞÖmA
s‹ý_Rô€Ë©Tß!îÞàѰހ}gkÛ-rÖÞôœ×Ûô?4½Á,íC?'l©']R¡¹]: ôVí	èiqàÌ/kÕc‡gz)*_‹†¹hÕD¬©·¡.b-NOaŽ1Ïrм*ïÊù«²1Ùô'ÌÑ>ÆÛî6¼ÑßÈ\Û$ë??ÿý2¢ÃøWJ·@*¢Ä"@›ŠbÁrH©P$ã‰Æˆú‡1ïD9"(B†ûP䊀Ü…J ]ƒ
RÃBøC#Q1Äñ}ÞývmšoÛofggvf'äÉ0Ã\û͏çyïE@*'žøé5Ò4Ò<q…gÂM4nRÝ%âiáÁ"CN­¡k/ÉUɶµò3Úx«ºŠøZô<·u]Êy†jµ8Å3Ûtqsô…FÞ6DÎm…rv˓½4OîJÁåHÒSÒߎõ'ËœÓ[E%{):AÄÓfY÷´dùÚ¸'sUJ8Cò#»´é}ØÛÈSª:—qGØA3rt)ÍTÈ»ÉÄÈ+қ%
"Ìõn¤¾rF*³|>Ozƒ4•4—<m¹8+6wî¢þ	/­¾yuÏ9Ö=-‰¾vòÕÇrU²ìkMýI7Kõ£Dy±'}ÌI˜Û0£#אoȹHý‹ç¶q¤gIKŽÐŠIErŽ+'#'Ýs,i<é=ö´«b!uôOxÚ~ê"ìi䩵}f:6§™bíÍGrU²%C[úžv²–è}uó\Cè	ÜIo*å™Û¹#lu<ÃF¼Íÿˆw%7ÈÓ1ÒãF˜|Hn–,b¾{QÎh螊?‰ÛËÌ/<m¥'<4Ú=¿+žàx®h±öÎè\•<Ú]Š÷NßޝÛà9ðžuâgé\ñ+ñö7óöºœ¿ÆJ¦ÆH=-}™ù²<~6S\cDv®§î¹M|›ÓŽå-´îiN°6aT®J–X³êÛɔ¬©®iÆÛj?ÉäNJÝp‡žޖ‰sÌË,ÊAtI0÷–ì¨ãe¾Ž—>†.1'4]ü+>ˆRò³•â4π[‰3pŒ¬F÷D/qd­,²vjÊÈ\•|Úî:&Ágëîþ 5¼¦ò†Ï9Kw‹ƒb‹¨æވ<-%ÞfS_€WM"¾5¡'Ð#¦É¾ù)yášÏVˆzæÜbŒd窌ãó[Õ
š'冧é²vúý;ªäxõ!k',Å=Wž±#Æx?-yöšC,Á·àu˜û±EoE×,%ƖPö®§èº0çññ
sŽ9;)³-¯‹
¿W‹µ†wTÉw¬µ´žñÎméµpÿºS³Ð¥ÈºbMW‡ˆ·*æ
ü`öZD́)pÕŽÃËʨo®§~?C8(g4ÎNÊêðàÉ¡¤þ_laÝt©Ÿ]ÒA%ß±fÖ×l|<çXþüVUËDEöfr¤Ýô§œ¸©ä‰,­¤^¹'¼la‹ž‰ã`r#‡ùœÁyFCïDvRV›e#aÆ,øڙyC;¨""jö7Çó»¹H2çðx²™w¸õWÌÛ.â
ül5ìY눩µÄ]T`lGænœ›ðEðZÙiM$;£}À&f'ékgÜÛ^%ßùšSŠóMà=ÇoŸ›Ys벌ÊÜoàüì ŽÀruqòǑ¹8¹‰NÎÀ-øEF·ø.	¼·®_è0rvIq•|˚YŸMô¾QOÈFO@–"ûŽtøBò¶"û$:Ãbj»8Lªàm"±ô¯ûþçŒ8¯ÈÎÚ>3SÂÓ´Y[YÔ^%_²f6Óm~FÝ )Yð¢£ÝeDx[Oül3¾fS඗÷𷝢<s[$7)qxEv†‹&9³6ë¥ÃÈÏkå¨äK֚[['¸¦ãu}g´F/=ÚuiFUçÕþŽ'ǁ9øWL´ãèð3pNk{ÎÎÔîvòÕÌýt9·¾ŽJ¾gÍ%®áEè¥à
3WñŽŽä|ÉÌ!''­ð»Š6ùxåkcœaæãì¤Lv33-±¶¹_;•֒Ç<	ˆ,ŒñFó>3G¹
¾°Å>Ž3gäƒà×!‹›eÁÎü×¼V‹µ­}Û©"V¬Å›×š~¿æÖބ?"‹&†¥ÈBðŽª»,g搫UËoiÇÙÏ
"3g§êy‰2•gº¬ß}W[•|ÏZsžŒù­É³¹'P–Ööœ#y[œ~	¶¢'çÅ8#.'áÁ"C®¯UÖö¶QÉ÷¬©xs²+бÚþÓ[Gy;^0¯ÕѼRf+*0ˆãè®8/nvzd^»P^ØF¥´`­1ñö"Å2²"<Š³"²¾…ylEãù~ΐN÷¿U‡'‹Gzf«"6¬Åc$YL7ù–ð*æ
þÿ[äs¼ƒ'3ÎN›ù°SZ¬Õܑ­RÚ°æô7kúòªºS³0‹1oà+*pF'Ç°®§¥2kµ=B*¬9÷ÌpÑ$æý
ÌI1gtÜTv¦0k
ß"TJÖâ±àÏQֈ%žÝàoÔ˜9li?Ö;ýÀÚIbK!ß³æä7Ó`$Ææ7xr"öµ³Ó¬Õçg©äKÖÜúfšÏM1_RZÙéöšš`íÒùî!•Ö\x.΅¿sÌYK׺½žfYk ¶ò%kf¿»Óϧç,Õá̃¬5\éRÉ·¬é~{·87s¾Ûkg–µßº…Tò5kvúš™\6ã©nzo'X»ô;e¦B¾cÍÊ÷vƒ3»ß1•X»šŸ­'ïX3ËF*¾"ÇYk¸–Ÿ­'ïXsú;6½‡•Œôk×ok£'ïX3Ë]ª¼‡Ûïh'kF¶*ùŽ5·g«cÃÖz¶SÉW¬|¥k¿wæ¨ä+ÖìdÏíwOQé0rÁèÝQ%O³ævV¦!·:Œœ7útRÉÓ¬y7·×ÇÖÎýnQÉÓ¬¹ÍQò¦ÃÈYc`W•ÖÖìf­Þ¸'_%Ï°æ6/Ú¬ýdî¡Rʳæ6i̕UÖNŽTJyּ̡Ûëãk?÷õQɓ¬¹ÍPÀZ³úÁ:P¥€µ€3»Y;a¢''Yó
o>dO‡'°q‰JžbÍm^Þ´X«3JF¨ä)ּƝÛkäknja£U²ÄšÛß0`#¥Y«1†?¡RÊøšÛœ<ÛÆZ¥ñÀ3*™e-P @
Ô¼þ`ó2u
endstream
endobj
62 0 obj
<</BitsPerComponent 8/ColorSpace/DeviceCMYK/DecodeParms<</BitsPerComponent 4/Colors 4/Columns 154>>/Filter/FlateDecode/Height 133/Intent/RelativeColorimetric/Length 5629/Name/X/SMask 72 0 R/Subtype/Image/Type/XObject/Width 154>>stream
H‰ì×
•Uðç²×]BW¥ZiD†4ˆR%-šr&3'¢ÂHÌ,Í¡ÌPPQ0Y`؈¯uYùpa×ý`wù؜ҘF'Ì1§qÒÑÇíùŸ{ÎÝwïœÝ}?Îûqï¾ãü‡ë~Ü}Ï9¿û<Ï©®¬8W'Nœ89š"gô©|eVÿ@ö:mƎ'þù¤Kì,"Ö²À›#ƒ'¤Kì,ÖÂ^ŸAgõë ]\;òsž
g'këqélh¢ƒt1RÏr|=yÊ¡ý°cä³ÔAºÄÎBv–EûbÇÈlJ—ÀåÀ~û²ö°×aÈÙUlJ—ØYœ…½ƒÎƲ)]9³»O}¥§d>cŽ¯ÙŽ'ëؔ.±3ƒÎzû¹°Ÿ7g7°)]÷MӆrÅ^.¬Á€³IlJÏóYìÌù>"ý¬NÖdymÇÈÍlJ#÷?ͅ½×nÎ$ÛÒݳgœ…#·²)]ŒÎg±³ðŸÃÉó:Œ#"Ù".¾Üü2¤Õ¾ð™ðÁÙT6¥K쬏9siÌ®³ilJWÎ2Ÿ×ï}	ٛ¿ï÷ú3­¼—vŒÌ`SºøVÏr%a:Ó՞ ÖâÒÙÝlJ—Ø™Á3éÍK"â¢Ú1òK6¥Kì,gُÎ~Ŧt‰ôÖÛû"½–îžÉ`=û-›Ò%v³¨$óY
÷Í9lJ—ØYsf]—Ã5Ú12Mé;óÙYwßsßÜ̞6Í§H—Ø™Ësҝ—ÛsŒÂz9[Hï".±³8k?>³#‹é]Ò%væâlzۯάŽÃ^"CgKé_¤Kì,b΂ô僳åô&é⻳¨ôˆlqÆþd÷àl#]bgù'­ËŽ'5ô麳(íµ‰32±æ¨¬Å…³R:KºÄ΂©ž×oztïg žm¤WI—ØYn²tívŒl¢WH—ø¾qgAí¯µnzp¶™N".±³,pfj¯{z/ێ'mÔNºÄβĜµæDØY9µ.žœ™X{T¶« ë™uÛ1²ƒŽ'.q=ËgX¿#;©™t‰e‰³X³cd5'.qßÌo¦×¢û^/k¶cd/Փ.Žœq^öτlðÔçۅ³}TKºÄβÔYû"±.;FP5é)g^öÏ´‰\tæѧ#/ÒAÒÅñ|f=WëšÃ®g±3ß­Ù1r˜«—.'©g^?oA˜ˆ'3·kÈY
=Oº8vÖÝú²ì³™µÎBÜ;;FjU¤KdêY{†‰°fÇH]réIgQ­g½=s³ë¬¡%éâøÐÝú²iîAQޏΎ,']\9Ó­5›öÒïgêÃη'.Fúf¶í£ÏÖjš#MC6".'pôžÅÎ|sÖ\ô'Ò¥ÏßB8¯H}–;;úÉ
	]ú¼³ˆÕŒÀ×nØÙ±ËÖ%t	ÜY>zûû¹nÉÉ~vvü3«º"æÌ­Ÿµ_?Gä$þÿP~*sÚÇÍËWi»ö'óÒùò£é´~i~²mì©ŒYNë腝¹úI},?cý]õ~â½-ËúÖgÏ*Ÿû¤\‹XÏ«-gÅ+ºdM=ó˙å™Ú•-«%åÇj&ícQ²õóH¶ŽZ'×:ò)NI^ˈey-W,ï×ò¹œ•ýN\Î)^ß鵩+M»´kð5|Oü\ñª~¿+Þá÷Ä{‹¿ƒàofU&Ó­þ°¦Lk.öՎ'¼n]"ëÌMíóRáÌbLÙJ»²x–°Êаu)3C×óÌ[–h¾˜Sôgjºp5}b;5–SãÀtd@%5ì¤úäžÎäï_Ã÷Ÿ¡¦ÁÛÅïàw^¼)q"ßs´Õ#,¦
ƒOuµw¨ƒVo9k¹riž.'s–iÁgºç¶:ÃùX	_%¢NuÚêtÂÔàíÂ
ÌÔçïŽjóöÒK´Ÿjè:L‡è Usðµ"xý"ç°újbÕ%«ÄïÂ|ÂiӐ­Ô\´™š…»2én4·B˜ëâ
ώÏJÀÎZG-ÎÓ%r΂è›Ý¼¯è›Ò™ÕXª~¥|á|Q_pÞʖrpÒiª†…ÕÑ^j ç¨‰ž¥£´ƒZ¨'Ú©œN‰àu% ]ü½çèí£z: üU‹÷¨æwx)ñ¼Å]…ø›0‡ZëioÂZIښ襼1«ØW[κ™?#í,óçýrfùœIg蓨cʘê‰Ê—¬YðpHÚÚ'\vvPmcO[è•Ñ«´žþNëèuZKoˆü'_o¤×hý•¶Òi¶—r·›š©ŠßgÚÜAQE­cÓÂ÷WÑ[Ù=¬‰¹ÖP•3Ô³îj™ξøxRGÎzrb žtûó¦j™¿3ó?ú&Ÿ•ªe8GQÇ,Æê`ŒëtÁ'òõ,uj»)c?¥lëiz"VÐ[´"þM‹é?œ÷D–лTBoÓJú§p·þÆæþÂæ^µV«ø=•7ÔJQßx®COýTÖ5|ÐC•3ôMÔgS}Ž1shézæGÿ´ñ~íã爻›t†:¡jÎç‹:†ú'Þ†9µ&žáú¥|¡nÁl-¤è1ꠇ8³8Êàõ\Î|úˆ±»elq56Qã¶	o¨oMÜë;k›²Æó è¡¨i|G°:ëµgúà¬}ÜÃùº8®g&¬"áˉ3Ô4ôNÙ7•31"q-kè_)zeªŽÕc˜½Ðó6sÜ@g¹~c3oÓïé}áž~͹‡s7ç.¼¾ógŽðö±¨w+d}C¯…[Ô6ôRÔLX«–=uöñH;Ã|Æ}¿×Z懳	|—ÒÄX=Ëo6ßOÜÐ;qà³KÕ³M	ÔÔÔ2Õ+QÇ*"±WDZÅ=r	×0Ô¨Ùlg¦4u;g*g²%S8?âL—ámg!ýW8]Ã^1¿m•ÖpŸÀÝu=æ»8Ã|¦zfOs™_Î&>X ‹±ùÌ/S¦kš]gª¦qmÀÙ©z&œqÏĜt€µavB_ƒÌVOKcè¢>¡VÝ!}Ýƹ™ó
Î$¼¾…ó]éí.Y÷Ö> åÜGQ×R=ô"0­ú'¬ãNº"¥æ3îó¨e˜1Mnm¹éþºD¶ž90á‡3aç4qïY'‡ZqÔ⬚•¡®`n*çóÇ옯Їic?–u¾nâŒç\Ã+ƒ×¤¹[d}SÖP×0³aÆÃ==¦q×P½S8C=ãùý]Ìfvk™ξ~ÿ]\;3]Û¸0íÁ™¡¦/^%ÏRÎrϬãúÒ,fõ<G¡_b¶'û938ߓÆn¦®âŒâŒÁëќë87Jk?"sÛï8sïÅ=BÕ4Ü3Ð;•³†'ÔtáB½U=ÓÖ\旳oÎ<_Çμø²þ®Öv¦jšê¨¨!¨gp†ù‹è™gyvKÌU³ä¬5U›(kLs†%:èR¼.ý]#­Ý&g¹™ò.º˜kÚj6˸kì–ÎÐ7qÀ܈z‹ZÖ6ö‰¤'Ï·Kg§¾uïùºDj>ÓÙ
±oªˆ9ï8Ëæ¢ÍâlQKö[œ•Òë\wÞ³?fù;åÌõ5éGƒ­¢¼º(™ú÷'~tY¿"µ/Ⱦ
›ß—5m¶¼¬Î^ëâ÷€ÆÜ3ËR=Ói-óÃÙw~>P—x>³ñ;<ëàQÓԌ†3>@µ¢oÂÙ:v†ùÿQY‡n—=ðzÙ‡KcCØÖ 6vA~*ƒ¤7Ôµ²îM'5m†ì¸S`FÃ=ÎÐ7ñ³.Y%îLJ•¦æîñ®?ۆœ½<ùgèâٙ"gÂIÎTM㾄3Å<"3FMAmÙ*ëœa6»WÞQ—ÆɞøéDªv)cdðö>%kÚhÙgoåLçü†ƒ	g¨g˜Ïª¨Ȧõù{DÏLÕ²Eɓvg?M¹³P—À糞ο§¯›²êvŸùg1§áLQÓ0£âÿªøî‡{@)ß•³{ä,¯œ'3Y'¬e4Î.'ή–ξ-kbÊÙÇÂYÏg¸oîcg˜Íî cC×'ZG–8ŸËür6õŽB]<;s[Ϻ«‹QuÆÁìƒ3Å}½³†^g^Á½µf©tvŸõwYÜ7wñ<x€•©žy¢xM=ÝU-óÁÙéiÓuqåÌKMÓ¹êiݦ{¯Ç÷S5
½³6o/w¯ªäSÆ–ñ}ó±Œùl'´sy/óîj>SwN5Ÿá°†Îñx&=›5ì$ÔUÌem×>ržŸ¾9ûÉ´Aº8¾oêj‹WsNyñæq¿EMã9
ý
g}˜O}·¸œwÂô¡¸oΐV¾šqßDMƒ«!2x
ÃeÝ'ëàyߜÃYLï‰ùoJ÷̦Á©ù_Ô2"ûíÕÙO0XWÎt5ȧϐñx¦¶1'èW8kÜ;÷òٗ³µôabÛøgª4ƒ;çΕÒjl!ä±QÒ㍲gN"u÷×¥ô÷eÌf-âîñöË<6ª*ŒâwÚaZ(mÑ@PB°Ð€¬'EeßÜ JLˆ&&Ƙh"Æ1j'P•¢ @SŒBTÀ
ÊR*•¥…î"'"V£MT\'ñ;wî4
ù¦ó–yïͼy!‡¾f¦ï¾wï/眯Â0äeC7¦ò2ƒï®…'s/,Ìæd¸ŸÝüÓÌ{ÙÉ`,ا.OÍUvÖʎV ²óåióI«üÌSž5¬‹Fª\c3UւÏçUf®Ên¿"o¢¢ÿ×
Úl«—iå¬å¥ٜ›7oÎÝh\ÄgÊÓpÖð´cDÚ!š;Á<m
yÚ25 §Í#Í&MW¹8^1—§øš¬òu®ÊKð¹˜ô&iyfYÌÈLôÿê¾ÅÂp/3ñÞZù~ɼlN¦çŽ3ïÆÝ3–9Üݽôܓ¾‹Ù³¦ÿvÎ><`&,?SwÿKæç‹jn\¨ò¼= òq†ºž£ºÜ"Š±%¤eª—ÛpÿG"^†^Fóˆa¾¬äìÕDz9™šôæ§V¶ºc×Ä>Eô3n
-ž–·24{véiðägˆµ¿e_¬rðiÅÒã*Oç+þž"=CZ¤ò6_1ö!åe±h'™ŽÁsxÆ<3Õ>ÓÃÙù¥s³9žŒø†‰wŒêEf83ñ<cÞõÃÓN÷ÜGnS&}g·8+¶‰VÙÕàkùªk½¬fÈç"o=«®)ƒÿ¡Û­¿ÉN¶]uä%8®Ê*˜?Ùvæ¥.Ζ?šÍIwnFòƒxÝœ'š'æ0÷ə€æÀ2J7ôu̟ð5ðò¸.V‰'7øÛ늻×[Ë_kÄb½øUf%ò7ÄX…ìÈËÚÛ·úÀµå{d'³oÏÉædš³xP,ýÌÀY`îƒÏÈüL=,¾'$k»kàf#y|
þ¶Jü#Vˆÿ¤ÀøZG,"k·ˆ6bì¼ÌßRš-ÐÉÀoM¿¾†Ü'»»¿^Î.®~(‹"+8Ó³—Ü÷£Ý/ʽ›'-OkµÖ¿©Ì,'‡>òµfÙ±¶ÒÌÞ
Éߐ§"
ˆ­M¢ƒ>k"L¢óï¥yŒÁÁXÕ-»d^'göY´¼‡YÎèï5qöÞýYœ\ÇY´ý´h
Ì
¹…2?O¥}NŽv"|í¤d­D4?ßQߺ {ÛqUúTD×à†^fìkJ˾/<RæåÈu©Èh³žd"1­œý°~f&'[9‹å9eÎB†Ñà;Õ}‹X;.¾"
n>£™Y¸‹X'g+?äë^bq?1y˜úƒ'¢"aÆ@ÿkºç­Ž0¦"³K…Ó29¹ÒϺc"ÒwbÀº|§v@'¯ê֏EEà d
܀Ÿ4‹'7x¸
©žøª¡9õ49`¹8JY	Æ0¿V÷Ý)ê¦tv§8SÒÂHëæ)½9¹'3;r3ºMãVùá?È:dú2]9
Þào‡"JÅ)š)ËeŸ+£ÿ'•§Ò÷	pZ7°H楩îodLøYë¶É½9âŒ;3'2ÑÈÞZ̵œ	ŸƒC]­2óékð¨oˆ#x˜BžBø½ŒþÁ÷N¦–†£ÞNe^·š¸ˆ5[Ì=µ0ryç"N®ô3=œYpVèRð¡ºA›}ÕÄ|
}­Ü_*½
L#ÊB:"=¾‡¬c5ý·ùÂy	n#ž´÷‰…º¬£…'+{îÍà"ôœ™½_"³'ù9lCjÝÀ->øZUŸ=²×WöK¦Ê•p
«Ì,'Y	Æêr6…òÒÉîoÐÏ®ìËëÅ)©8³'¿æ‰ùøQCnA
z–d8BŽ'7xT™ñ©€ßaF•Œ''ÏƱ«ýg¦,µçÝ5zºF~<pw'×sfçp"ǯð7ŽZ«X#_#Žjú퐼!¥èي>ÖÉؘwü–t-ûÓÍ~iâìðØ^œ\ϙֽ¶àÌäL@¾Ô8üýTô-°žjúo—þ&EìÕ(
1F½\'OËÞÑÄ,¡…'«GG§sJ*άð³h3ùü	¬Á×ês>ò7d©ñ̡ױÝߦfš³ã£zrJ
Îb´ÏF8CǒùfxWa5䒐•Ôûá}2/ìúf9k«'ÎÉ՜ÅxŸ®ƒ™>%YOÃק'-ɱ'³ó%º¿]Ï­Sš8«"®¹š3-,رýŸêd
\7(ÌXÞJ?x´Â‡lå¬~X€SÒp‰»Ø&Ÿ'_IÖ0€7ה«óe'svíÛ¡NIə祁™Ÿ`¼¼Iæc͓ÞÐîeqÌY{ːœ\əUçe²s7"§I֐¡à
3¾¿Ó{g–³Ä#3{׳֩®ŒÅ¡‡éæ¬uH€"+9ÓÜë5âK*ŽçKCœµå8yœ9°.}.}
Œ9ùŒpÖñSN€"Ç™3œ9þ|VqöqÅȵœÅºŸéí|Z×ug׉+F®ãLVqK9½Ÿ:9kÿ='"ë8ÓËD<=‹8ë¸qG'Wr¦ç|c¹^ן±`,9kÿwH:'Wrfõ9j¹g'æfG07"Ç™ÆûEûŒó3#Ï"àœµ‡÷â"ôœ¹ÐwœäìZpD'Wrf†5§Ÿ;Ž¥…'«ÁÑYœ–3'<+ÉÙÕÆÙ]}8%$gNs"d|éáìJp\_N	ÉY"ñæôÙÌÙå`Þmœâž³ðYu=7§Ùñ8‹¨KÁûqŠ{κã/'äô~ÙÄÙÅà"\N	əÓÌ$_z8;œt'§"ä,QXszà¬%8u§"å,xszoàì\pZ§"ãÌiv'"1­œ
NŸÌ)a8sš=Mœ	ΘÎÉãÌã,–œ5gÍæwœ9͂Ǔ)΃³ádˆ3§ÏÑã#n9«
>¸€SÜùY49Íb3¬³žà¤‡3Ož<yòäɯÿô
endstream
endobj
63 0 obj
<</BitsPerComponent 8/ColorSpace/DeviceCMYK/DecodeParms<</BitsPerComponent 4/Colors 4/Columns 132>>/Filter/FlateDecode/Height 134/Intent/RelativeColorimetric/Length 7656/Name/X/SMask 73 0 R/Subtype/Image/Type/XObject/Width 132>>stream
H‰ì—}lÔõÇ?׫­"¡ƒlŒ*"ÑS˜[4:5n¨˜±
c6%s":ƒ€ãQžG¡t%Ú®@m'>H…ÖV úmé>`P¶˜-'‹Y#>-ËØûýù}~ן·ki{×»kéïäz½»ßÝïóú¾ßïOUqṪ
h@ê@oÌX'|Yiæâ+£¦XÿÖ.ê²æa€‰bÅE¬_¸<œ›ðx‰õ÷4'º/}ýÞõ÷ß.ýM>8ÀÃ<Ē•XÿŽžòÉßÞGïG¯rÑ8é5ú›ú9!yèÊï¶÷ºe©£éÏ%©¦-¨í¦W¨¦®TµNYØ6yMbۍkU­7¬kפõmLl½þŽ&nö4a«#÷o÷5ßãýû\÷Z*\[¿ƒ}÷ûy¿sàwØïŠq0ß°yè'Í^ï¹;ow>ÞÙb¦-ãÓü-×mKh—'Ðœ''Ð4v»¯iL¦¯it"í;9
úÖ_ãÈ_ãj·¯aø¡øXŸÃÿø¾–ïáû›Ç¾èãçQ-ãÒô¸V€£`vŒ™'..¢Êƒûúp?/Lïê6xÏWx0¾Â€Î>ÕæžîÌÝfî5g\?,Oê¯~INÙ'ÇK]ò~©M*'šÄRí/•c¾Wå˜T8Âc>W‹ÿñ5|ý‰ÁEúÞú¡ùúY7df§ñ'åðâr¢Œ¤Î÷õrá2ës5uÆC7¸ç=ã™
x'ëpVqfÏp¡Ô]Y¬³­I,•j_¹•×äu©"ÃR5R&uR
•©jõ9þ¯¯¬ÒW:œð3j"#…z
^K=…~â²?
pAnÍ34Wú#¡|¥«þÐ
_QÀ½xƒ‡õíµŸ}Ì¿Ja®•:ßr̹TŽË+Ò ÅrR
å"ì•·$OކN«òñx¯¼)EÒ"/ã5¥^9©j%ƒ,')òAÎè5.®o(®_à»:LñÜú¢º'?äA="ˆí8{¼ßd¡ÁX ŸÓÚ98l'»Zçé2°pæ»å]Ù)',ù»¼ ç óªLùÏýMvÉYɕw"ró²4*åðCH–# ÃË=£Ý/&è]ü®šðˆýÉByBwý!"ÇtÐexŽ´?xxà¹ãýn°P žÀÜçŒèóä€P'9ò¬çc®ՙ§Ë‡²Yþ%äSY+_@ÿV­"/ñÜقÿeà5™àÅaã´úF±4+[dŒ\Tª_Th–GrÙ0<W˜ô/~Wí›.È¿¸9ËáÎ=}²ï×NÉþăzÎ$Ï&çA78¢,Ôà,W¿ß‡r–ô‡ƒ€ƒOd
f¿\.ÊbhôŒ‰—B+!²ár'¥\¼§ÙâúE©å™`
øzgƒëÊCªæ}îÔôe±?ÇQöƒHóð†ë¼§8kÍèkšÈkÇè<8·,áÓësà	ôÿõƒåyùü³~zú
ô4ÏÄǏÙÿÈ™¡l'ÊväÉy>sF½'¼±8>qþT¦>EFÙ1<¸ý¡§ÞБ§ÆƒbÁƒy"fî­úƒËºÏ%½}>γK_àÜ\6ÁVa¶ÏBlîs¡¡ŸA÷™øxôKce¡ù™`¾lG× {ðÙð	æQ9®Ék»ádÆiíãD_£¿õÛÞÐM¯ˆ¼ŽöJf:»æ…ñÀù:&rÞð
:û3"só²À,˜o³ž
Ý
Ý͂f˜øøè^cežyÅh5¼%՘`a/¥4¨òð@`Ðý'ÞûÆ«¢Ü\ÑoyoÙ!x¯™Ñ¥ê×ì
%èzôæûó
æH_ø±pŸÍœó¿šìÑThšqñècâIó‰uò¹¤¡ƒ°gÒ¸¯pïx
,²Ë''/rt¿`¾9ÞFoèà|"|.šü_'Ê<x=¢	'÷œg'þ@ÊÁ³'»Ïoò~½|¦}aÍÕeaºÍ"4ºÖÄÇ߇¦@·÷[v<Ñgè7ìì—ì(Ü7*¼<|<ŒÜٞ'Ü)BÍ¿øBÄyðôˆ–qéÚ!xk-/NêðgôžãçÍ…²ùÞ
Ý`³};ᢌò9
¥'äåG–+¿€‡ž3à¾Ê…ì•šì"Ãò"yFãweŽùìú£?¸¹Á]½²iL&:D®Ô%ï׳Yàá´ú9³b…k×fY&Îþ°ðÄ‹2Ôïh8ô͇"‰–·™GüÚ:ó'M>Ò^ÉAØ]Ø'¹o6¸YŽ7ôÐ?cÎGxàyÓ?ÖÌ\¤³àL˜ôòÀ}`™eÅ\;ç?4o`6ÐÈÀUàákIŽø˜LÐ3¾k1ÓXšg{*3ƒûg¶òð–vØà 'ûæ‰!Bߢioè©7t‡X²àý±âÁõˆ	©~ú2óºÚ_ª;³<ßÃýý·ž¬˜fýà;>gî.ƒL||u¢ãc2tuQîŸ+úû÷‹J$–vd}‹þÅl‹Æýˆ!®G°Wrï¬Mb‡¨Ô®Ïe¡?xy˜ãáa¢e…Ëà ®òð0ÉÃÃÜ vÉYÝeʤ$d…î˜ì
Q¸·qÅFYîfÚþ‰}ŽþÌÌ8ŠÌ(Çl
±òìrfÜ-žáœ5gʆZ‡H1`ÿ¼×üÁÝ1ØUs°_I‹îšÕ¾rÝ+èWì
=ò†Hq+&bé&z»}º&±TgS,Í:«m˜û䓶Üm;¤·?KÝèãmïœåéÏXŸÌÀ~±GÎh_aN1+Gìö5§dhoˆ©/D›
ïçǘÝ?á#s|ôkf;gµ]Îë¾É>Ͷ]á–c‰áþv]c»çµæ#Ó¡;,o¸³.6ȧò>ÛíÜmèOM£oèñ~Ù×Xþü8ðõdµzüš{F™Ôé¬Ø)7ÊYŠη̸ša{™H±.1Ê4Úùù±'+˜;Ë¡Tô'lô"iÓ—¾Dâ¾ÓcoèMz›‡8Êõˆé˒]`¯¤y2cµüW÷ÄG û­GÌ°yO2.˜
߃®·<™f9qqô´Z'ŸÃw>"Ýò®ú÷
z;L뤍—WNtô;.ñ{z›Šç'qbHú7÷î/Ê9Ùàž±À:Àlcb–íäbªéf{î6ësŒ£§Í¶¢£Òè?ì®ô#zƒö†©+¯ˆ;bÅD$yèkqÿœ¸Ùß8Âõˆ£èz'õ³G¬—Ï47Ø|²Žx—õÎÿvèNãà§ÐÏ­3,46É'šAyrZJÐ#é
uÉû¢§Þ
"ͅw.¡žÇ:»7Áu)˜¼ÆéW¿¤Á±Oޔ]rVґëäKeb¡ÍùWÆÅæԃÆÁÃÖ9~-S.èNA¾¸c–㳫ýeÒ0l¯´\·-¡í¦ñë
½ÍE7s#yáŠýžçÕÙ5kÿw™à<Ù/Wa¾‹¡§ Ç­<jšo½'î'›åc͝e¡Ys'¼';Ý)Ðgû½'
ÝümÑäç"çµax®Ô&:ݒ½yO&˜[°¬•/48óg­+.2NØ5VYwÜ*)ô…9¥žÃ–™ÄþÚ2>Íßãý²¯æE˜¿+š<¨GxöOzºÃD½ú皅ð'x÷Æ
ðæù È³!
½'{D¶¼/{ä|¡MJá5.äM÷KdToÝ·>ÏDwò¢³÷tæKÁ¯	q=wÿäÈ]°ÚW.‡¤Z}bÎx®¼#;0çLùr^»Eš)ÐCØé'ìŽ.äª&±Ts"Ð!o
ú¡¾c<±o<Déú<·Ì
îìG±rçàʐü؍s¿KÞS6¸CR|œƒçrÁÁ^ø	w"RdÄ8½FYg̉SӖ'…uïcÅC¸lt÷½—ò‡^æϽÏoӘLŸv	x<;à!9¦gs."Wz@®)OÞÖ®AOàNY†îH_ Ç+ò՜'' 2Ö³ì+4«¨øCˆßÌnÙ:!ÕÏ ~h>˜(1Ÿ¨Ò^Á™ƒ
zÅÇ%Èî%Rƒ¶P`\±—3fÒÿÝß¾ä
ý‡®Ís¬¹]€^ϝã&]	ÿg§àù§_41Ê!f»ã1ß«R—¼_ê‡å9½¤uÊêð:d¼2Ò^::Á;y_¯óÐÉïÒn‰óL0Ÿàœ«@{ý'ówT¥žPfªý¥êô²@®Ún\›ø?öË?6Ê»ŽãÎ×^»s1ÌY"¶+µt"ßE µ@A%ÀD"	›¸ÅÉæÔ¹hãŒÉÔH¶èâb\fŒ†dÎeÉB]HA"Ú^[h¯½»Þ]4ò°˜e>~^Ÿçù>}z\Û»ö¹ÞQ÷Ç'<<}îžç¹Ïëó~¿?×»›L'òæ‡Üg™êsðÎo¬xâC̵f‰¹6Ì<»ZA®€
»þ¬þ€ŽàH3CóÏ>˜7Cæ>K¥Ï~™8ÈËC)ï5Á»«oÈNpþö_ßB&<óáÞÇ.ŠVÐû¿:Å1¬œ¿¨qö£¿¹E3ÃÂ#`g)ú7/wß+'¢xÈý-}âD³¥øƅú_¼Ÿ|©LH¿O‡ÿ \ ÔéÐu§$;¢h
Á"fșš£JeÁ‡ž"%Oæ)r šo3!:!³vîï"|AKŽñ"s~"ážÊòܕĂOU4~<cž÷Öl)sÎJ€	úŽ ZÂÙQYnàÇ͐7S+"…)ñPÂßÚö+ô›lxˆ–pp~þ/u—ÐÌ ,ä͐³¡ÊÀB¥ñpyí!Û7Òw´Âԅz)‡®q}¢Ü½›ELÌx~˜ä7`ޙ{e'¾Ë.JNЬ Œàú7á~ÊÞ³YÄBYx˜Œù?sï2Aÿá'rX`·œµ>QfÆ*'‡\&dîßXñ"Í.(9†x¹4›µÁ§ÞÞ4úPÀ»ªoÀý."
ñeaõ÷¦¦
ë¾3Zju~;xyã·ìÚôÑúÜ£5T×æ¯ßX[	™êÞvЮ»¾6ǭ퍩.ïߜë½ß'ïæþZæ™ÌsòÌæù)óN>pã+¹÷ŸÿÌ¿2wÀ¥,|jÏååÀôÞÛoÓ[éY—é鎯†»w>îÞ}¸gÏWÂ=_ÚîÙ÷åpìÞ{"±ýûìºoo$öÀÝÑ؃{´zÚí=¸+Ú÷ðN-Ž9gþ®×òŠÏËwñ|w·Üƒ{é=)îÏs8yÙÉá#ãõÂ{Îs\V¿˜Œ/° ÇEû"¹Wc8ðö÷±½7=7ý4ý~tG´ï›_Œö=¶=ÚÿÝmÑþC[£ý‡·D¯üðóÑ«?úläꓛì'cÎ]ùÁfû¹¶ïñ/؟å;"™X./†—'6Fk`ÃËï4EVEóÀ50!þ Uãi¿£ª.÷Û0ûžþ›Þ÷›¾Ósé-}øÉÆÈà'ÎèàÏ×EŸéˆÄÕz~͜á߯
imÕ97ôÜÚpüÙö°^+Ÿá³†¾³NäÊ	ºb'gé1c˜@#àÁ‡\RÑ<˜,°P¬åÞÏ˃ÑÂÑGûUïéÌ2s­s/ó>ðӍÑÁ§7hÿéñðoWÏѾ¿¸rNâ•e¡ä«‹k'j	&_"MÉ9þ–xiEhø…•¡!ùLÜÃßÉw»lý0\8šÁ3ª^È3£Æ?ô|І²óPSàgÂbŽT{eÞЗùýUÇ=¨<e3@™ùýy¹ö?u¼%˜:¹°:õ·…Õ鋍U#—Ò]
£%çÒ竸&ù—;ƒð¢|ÈwÀú¡lgʆ膗4JµÂ0à†òƒ,TÞ~ç뻟<0G&?Àymp<¢÷'v&~¨' 2Ãê2×	£h½=Õy}A ÓSH_¹#ª
dRóÙtm¥Çœ¨·¯6à&u¢Y¹H[R£\à+h†0gôÂeBøԌÁ3ŠwhætxÐü`¼¢Xý,5ÞgòáÙ¦T…<§ü~š¼<myD\Œ&È«8ÐSՁ˜ÃÀßç2ÿš_•¹&\—ß®µKŽ³oɹË9¹&›kûêU7FÎ4U'.`/Á¸'ÃèÙE5Bž±Ç˃ÉÅÎL¥êƒïQh"Ì•æIüÂáA³££
ê¢ßC¹,HÿFDûé'3¯ À@öݺêŒÕÌX¤>UcÇ
Aþ¦×ú™xêÚ¢>òš1`"ntBžìŠF [è—ÍÃ;?ÀƒO9²¬<"RG
}ñ\ÕÉfšòÛÓ´O׬ 9ÐeáõQMÈþÃÑå`ApÄjž"²ߚ´–|dØZz•°–Íå܈ug>²ÿ­¯V½ø§G+ðSŽNwÜ2¡»žA†€aX½'é³¾Žá¡˜ß³Ð¾çöj¼ÞÍ4\K®Ä3$³ãÍ.'!ɏô"yÕ¼àx3=†éïˆÕ¢çCÖòÅ­•·X«j¯Z­R«ê9´Z?·V|Âæ¢)¤zVÈwÀDÚÑ	Í#'Ou'Œ‰>'#\ðò¤ñ
ïN1ü¢†JÅEŽ`ï"yÓý'ü`x^hn¬ÇÜ¢éäͅÙù/èÐÿ~kmsŸÕÖÒkµ/5Ź~ku£p1Í@G"	t&Ä;ðÕ|CôˆìJŽÕ\	²{Âlû¦øœ›|ž«²úE)˜(òYÔ3dÞ4Cˆ"̨z…ôÈÕ4žÜøŸújôß°@¿û¬µ-=V{k—ÕÑFu[üË9›‹5M0ÁgàH39Sv<ˆ4y|'ë†Í¢]=Æ+rµ¡Ôúà·oLÔo?4a<`îÐcöò~¡<#…2¤z}Zxx³®Šù&à°@¿¥ÿk.[ë:/Yë7]´6l6Å9¸ˆYíËa~ðÉ5캛ŒzÆØ1"Q͒'s؉È>ã¾w%ñàg_gŠŠ]Cr%ž.³o'åØ-"™Y͑Wî°s{¤£
äƒ~«m'aþ_°6ÜuÞêÜAq,ç¶Â×ôZmKð²†f‰wD#Ȗ'IFȕ'Y¹§ú…0©û…"\m(áïç«_ҏ\M𛩩<·h¯îž¢½N†`×#Oª_ìø|Fz‡Wè)ÚÀÜã
vµ6î¡8†˜àš˜õ™•F#tç¢ûªøùÄåA´‰§ÿð–(¹F÷Š\m(ÁLÎh~Èe!÷Ê¥^p<|¦#' Oâ¢Ê½Ói¼bM=v´a«aጵi/e˜€®A#ȗì)«%Šg!"aNý'<)Úd²ƒz…°šW*‡ÉzRâ÷™ÎskŽ WÊ<š1|´5Ä~'Ÿräš&ò¢—Â)Ãñ‡‡y¹< AhûfüÙö0¹V½mÌK֙ô]KŃw–‹aa:=ñ㽦sOÙát÷`ÇÃ3†ÅÇǖè~A~(™>ȓ¢Eš%…ErþÕ½ûÀÚà÷ï6ÓùÍýÐûréƒSF#˜KæÓdˆÔ©æ ;a¶TùA´æ`/.^‹øVì¾½vn`¿,åM¤Þßu*úpó@^Ó!žÝ'Á·~ã뙞ú€î†ìˆ~í–î,²Ë¦N
'%ã'[`m 7mfj&'ä!÷_¿«ïåÃs¡Íx6a<ƒ¡;†ø|öš0a5g\±>ÝÐkµ/¥ß]VÇzzÇp"çÛ¸ÆhCÊZ|«zÅ[²»¦æÒ]
Ôñ– y…½Bsäþ}¶6Ì Få…ô0÷;&úÛxçÊ©û'9B4'\I¶K¼²L=ƒ9Öy–¹6açÊՍÌ>ْÞSøÿrΰ@Žä3FðŠÌ@½Ä+Ø35G>¼ÓÎ
ù´¡<LuÞË]>iAŽèl{"yen™ß'K²g dÀwëªé«a +öYm-ôŸâ˜sh×$¬¥·'=Зì56œh²ÛâOª
'È2E¿§ß<äj@±úàW?gš‡ÜïA#dÇëuvO͕ŽFh®L×VÑO{×h
¡ÿdæŸLǜÃW¸Æe"Y$Mn™|u±jÃÕ'7Ezî²sƒÙ/gp&ÇðPÌožï9§ÓÃÉÞ»T<Lô]²ê®!9_5ÂÉôO}Ãa"óNxǂ ½f‡D/Ö²¹Ç6‹Â\?™7ëªðöWwǔÌ:x¤S÷\rÃ
ÚPé<"Büú GôÞ2ºkHÿÒç«Ð	ô^÷Å붐é{Z²•Ñ'Üo?øŒpäfÙ[ð	2
:"±ß\^ïhC±³ã'>ÿ–¾V™xÐýSrNΣo†	Õ	ÙA³CµLÖæ'Ù×}Tz¯uÝ>øÙŽ`<'xiE/Â'ȐèQÞý²Ð÷ýá¡Ðw-Á}Ñn4ß oôoXfÚ0AÆ$À…zˆx·ÒiáE8@4;ÊgdvZ"!Ñ£rjô{<PdKÑðØw«¿Ó¿¡çֆÑyÍ'…	™wzÍì"²ñ:- k #ª	'GùLâååʂf†C[mŸ—Ìò>ráÇwæù»îŸ'ùñ
úG
‰cKjÈôz"\q±±
ÍÐ☜r
, -dÓÁ§6DÈøDìÞ{"ÜcÚ¾8äó7¥Ð‡B¾Kþß½í`ˆ¾Ñ?úÈÎÃG[Cì¢ô:y|Q0u¢Y5ƒJÊ1çTä²G\>ó?öË&·‰ ˆÂëvŽ'%;@€`@¡,‹Hˆ
ŠDbÁŽ Ä8Iœàù.¼¯p[VÀƒ=?]ÝÓ½xʸ3cÏt}óêÕâ‹XP¡ы¬Oȇ:{`Ÿþ°›ÿº¯˜"± y9žNß Ž0OXžø~ó:ï=57¿øq°'­)+püà¿>?˜^¾ºÏìB^íźð°¼>;ðäA
}ƒ:&ð‰Å·ÛSÞ{ãB~¬Ê
Ì&ðc¾@~Ôw0OWÛÔ®7֮Ϛ‡>¼h×=¿{²7{òæ}ƒH]	eÌÅ×;SjŽÀ†1À1èpX ‡œë;È©§÷ßí5Þ_ÓçÊC¿y²Íõ¯QGêy!&ðýËOöéæòòI½5æTˎKl¶Tï±>Ñç3v`![šž½+OÛ|—r?;|5¡®6sÀ"æÞ¸ þ&³/sc³"òÇù‹£	ùôôއÍÞÐ÷»²Å³eÍÃÐû×t<ž¾1#Kˆ	|b~üÌÞÿùÇÇÆF­)k˜/˜'"O·º¯¾yh¸¾HÚôØ«ûyëO¶´¾¡úRgòÄÏ·Ï­öæøh
^ŒåG®±>Á|ãYw8T<lóìzë_R¶´¾˜8z9ef€‹‹ui
1ÈÌMr(þKàaS
»zÀ¶lÈóÉÔyÅýC^°'ÖŒ…Ãד3õòh«ìA£ãah]ý}<Ÿyƒ,!&ÈԞyZ3_Ð9QûDÉùÁːfê|˜ÐÜa ŽYS~4š2d
MŒí|V-_"jO¦0qŒ/`!†7Tâô¦ßW¶¤oä	€
dÎñÞ§xðä`ë2˜'vù®Êƒ?#]"^@Ý©ÿ'‹‰÷‰Ñð£OìÂJ`'¬€8ΠOdÍC,Úx×P¤¹ÃþfÐ'*rÁùøD÷~‡˜LôqoÞ{U1ÙèrOÞ{S){D¸?ï=3¹!Ó÷¼<™ð~îʃ?ÞÏZyH"‹'øȎÏQYñP¨<Ň÷½'ª¤yðî²Uy¨,dÁƒwe"YrbÂ{ŸÆȃwM+#iðà]·Bëž,9³â½?¥ðà]çÊC:<x׸`'ä!7.FÆG2<x׳2'9òá½G1xðÞãZ¿´xBÞTæZñPUUUUUõ?ý`ãsŒÒ
endstream
endobj
64 0 obj
<</BitsPerComponent 8/ColorSpace/DeviceCMYK/DecodeParms<</BitsPerComponent 4/Colors 4/Columns 132>>/Filter/FlateDecode/Height 134/Intent/RelativeColorimetric/Length 4433/Name/X/SMask 74 0 R/Subtype/Image/Type/XObject/Width 132>>stream
H‰ì—}lÔõÇ?׫­"¡ƒlŒ*"ÑS˜[4:5n¨˜±
c6%s":ƒ€ãQžG¡t%Ú®@m'>H…ÖV úmé>`P¶˜-'‹Y#>-ËØûýù}~ן·ki{×»kéïäz½»ßÝïóú¾ßïOUqṪ
h@ê@oÌX'|Yiæâ+£¦XÿÖ.ê²æa€‰bÅE¬_¸<œ›ðx‰õ÷4'º/}ýÞõ÷ß.ýM>8ÀÃ<Ē•XÿŽžòÉßÞGïG¯rÑ8é5ú›ú9!yèÊï¶÷ºe©£éÏ%©¦-¨í¦W¨¦®TµNYØ6yMbۍkU­7¬kפõmLl½þŽ&nö4a«#÷o÷5ßãýû\÷Z*\[¿ƒ}÷ûy¿sàwØïŠq0ß°yè'Í^ï¹;ow>ÞÙb¦-ãÓü-×mKh—'Ðœ''Ð4v»¯iL¦¯it"í;9
úÖ_ãÈ_ãj·¯aø¡øXŸÃÿø¾–ïáû›Ç¾èãçQ-ãÒô¸V€£`vŒ™'..¢Êƒûúp?/Lïê6xÏWx0¾Â€Î>ÕæžîÌÝfî5g\?,Oê¯~INÙ'ÇK]ò~©M*'šÄRí/•c¾Wå˜T8Âc>W‹ÿñ5|ý‰ÁEúÞú¡ùúY7df§ñ'åðâr¢Œ¤Î÷õrá2ës5uÆC7¸ç=ã™
x'ëpVqfÏp¡Ô]Y¬³­I,•j_¹•×äu©"ÃR5R&uR
•©jõ9þ¯¯¬ÒW:œð3j"#…z
^K=…~â²?
pAnÍ34Wú#¡|¥«þÐ
_QÀ½xƒ‡õíµŸ}Ì¿Ja®•:ßr̹TŽË+Ò ÅrR
å"ì•·$OކN«òñx¯¼)EÒ"/ã5¥^9©j%ƒ,')òAÎè5.®o(®_à»:LñÜú¢º'?äA="ˆí8{¼ßd¡ÁX ŸÓÚ98l'»Zçé2°pæ»å]Ù)',ù»¼ ç óªLùÏýMvÉYɕw"ró²4*åðCH–# ÃË=£Ý/&è]ü®šðˆýÉByBwý!"ÇtÐexŽ´?xxà¹ãýn°P žÀÜçŒèóä€P'9ò¬çc®ՙ§Ë‡²Yþ%äSY+_@ÿV­"/ñÜقÿeà5™àÅaã´úF±4+[dŒ\Tª_Th–GrÙ0<W˜ô/~Wí›.È¿¸9ËáÎ=}²ï×NÉþăzÎ$Ï&çA78¢,Ôà,W¿ß‡r–ô‡ƒ€ƒOd
f¿\.ÊbhôŒ‰—B+!²ár'¥\¼§ÙâúE©å™`
øzgƒëÊCªæ}îÔôe±?ÇQöƒHóð†ë¼§8kÍèkšÈkÇè<8·,áÓësà	ôÿõƒåyùü³~zú
ô4ÏÄǏÙÿÈ™¡l'ÊväÉy>sF½'¼±8>qþT¦>EFÙ1<¸ý¡§ÞБ§ÆƒbÁƒy"fî­úƒËºÏ%½}>γK_àÜ\6ÁVa¶ÏBlîs¡¡ŸA÷™øxôKce¡ù™`¾lG× {ðÙð	æQ9®Ék»ádÆiíãD_£¿õÛÞÐM¯ˆ¼ŽöJf:»æ…ñÀù:&rÞð
:û3"só²À,˜o³ž
Ý
Ý͂f˜øøè^cežyÅh5¼%՘`a/¥4¨òð@`Ðý'ÞûÆ«¢Ü\ÑoyoÙ!x¯™Ñ¥ê×ì
%èzôæûó
æH_ø±pŸÍœó¿šìÑThšqñècâIó‰uò¹¤¡ƒ°gÒ¸¯pïx
,²Ë''/rt¿`¾9ÞFoèà|"|.šü_'Ê<x=¢	'÷œg'þ@ÊÁ³'»Ïoò~½|¦}aÍÕeaºÍ"4ºÖÄÇ߇¦@·÷[v<Ñgè7ìì—ì(Ü7*¼<|<ŒÜٞ'Ü)BÍ¿øBÄyðôˆ–qéÚ!xk-/NêðgôžãçÍ…²ùÞ
Ý`³};ᢌò9
¥'äåG–+¿€‡ž3à¾Ê…ì•šì"Ãò"yFãweŽùìú£?¸¹Á]½²iL&:D®Ô%ï׳Yàá´ú9³b…k×fY&Îþ°ðÄ‹2Ôïh8ô͇"‰–·™GüÚ:ó'M>Ò^ÉAØ]Ø'¹o6¸YŽ7ôÐ?cÎGxàyÓ?ÖÌ\¤³àL˜ôòÀ}`™eÅ\;ç?4o`6ÐÈÀUàákIŽø˜LÐ3¾k1ÓXšg{*3ƒûg¶òð–vØà 'ûæ‰!Bߢioè©7t‡X²àý±âÁõˆ	©~ú2óºÚ_ª;³<ßÃýý·ž¬˜fýà;>gî.ƒL||u¢ãc2tuQîŸ+úû÷‹J$–vd}‹þÅl‹Æýˆ!®G°Wrï¬Mb‡¨Ô®Ïe¡?xy˜ãáa¢e…Ëà ®òð0ÉÃÃÜ vÉYÝeʤ$d…î˜ì
Q¸·qÅFYîfÚþ‰}ŽþÌÌ8ŠÌ(Çl
±òìrfÜ-žáœ5gʆZ‡H1`ÿ¼×üÁÝ1ØUs°_I‹îšÕ¾rÝ+èWì
=ò†Hq+&bé&z»}º&±TgS,Í:«m˜û䓶Üm;¤·?KÝèãmïœåéÏXŸÌÀ~±GÎh_aN1+Gìö5§dhoˆ©/D›
ïçǘÝ?á#s|ôkf;gµ]Îë¾É>Ͷ]á–c‰áþv]c»çµæ#Ó¡;,o¸³.6ȧò>ÛíÜmèOM£oèñ~Ù×Xþü8ðõdµzüš{F™Ôé¬Ø)7ÊYŠη̸ša{™H±.1Ê4Úùù±'+˜;Ë¡Tô'lô"iÓ—¾Dâ¾ÓcoèMz›‡8Êõˆé˒]`¯¤y2cµüW÷ÄG û­GÌ°yO2.˜
߃®·<™f9qqô´Z'ŸÃw>"Ýò®ú÷
z;L뤍—WNtô;.ñ{z›Šç'qbHú7÷î/Ê9Ùàž±À:Àlcb–íäbªéf{î6ësŒ£§Í¶¢£Òè?ì®ô#zƒö†©+¯ˆ;bÅD$yèkqÿœ¸Ùß8Âõˆ£èz'õ³G¬—Ï47Ø|²Žx—õÎÿvèNãà§ÐÏ­3,46É'šAyrZJÐ#é
uÉû¢§Þ
"ͅw.¡žÇ:»7Áu)˜¼ÆéW¿¤Á±Oޔ]rVґëäKeb¡ÍùWÆÅæԃÆÁÃÖ9~-S.èNA¾¸c–㳫ýeÒ0l¯´\·-¡í¦ñë
½ÍE7s#yáŠýžçÕÙ5kÿw™à<Ù/Wa¾‹¡§ Ç­<jšo½'î'›åc͝e¡Ys'¼';Ý)Ðgû½'
ÝümÑäç"çµax®Ô&:ݒ½yO&˜[°¬•/48óg­+.2NØ5VYwÜ*)ô…9¥žÃ–™ÄþÚ2>Íßãý²¯æE˜¿+š<¨GxöOzºÃD½ú皅ð'x÷Æ
ðæù È³!
½'{D¶¼/{ä|¡MJá5.äM÷KdToÝ·>ÏDwò¢³÷tæKÁ¯	q=wÿäÈ]°ÚW.‡¤Z}bÎx®¼#;0çLùr^»Eš)ÐCØé'ìŽ.äª&±Ts"Ð!o
ú¡¾c<±o<Déú<·Ì
îìG±rçàʐü؍s¿KÞS6¸CR|œƒçrÁÁ^ø	w"RdÄ8½FYg̉SӖ'…uïcÅC¸lt÷½—ò‡^æϽÏoӘLŸv	x<;à!9¦gs."Wz@®)OÞÖ®AOàNY†îH_ Ç+ò՜'' 2Ö³ì+4«¨øCˆßÌnÙ:!ÕÏ ~h>˜(1Ÿ¨Ò^Á™ƒ
zÅÇ%Èî%Rƒ¶P`\±—3fÒÿÝß¾ä
ý‡®Ís¬¹]€^ϝã&]	ÿg§àù§_41Ê!f»ã1ß«R—¼_ê‡å9½¤uÊêð:d¼2Ò^::Á;y_¯óÐÉïÒn‰óL0Ÿàœ«@{ý'ówT¥žPfªý¥êô²@®Ún\›ø?ö략ª °ñ£'€MÁBH§müaŠÎB+ÁFÐÂʏ?`o‰!D'óν7–sÏç=o1ä7³3ÏîÎq×»`çDëüæ25Ïk¾:9½ƒ}­³ÄÑÆö<ÞpV`®€MüÐûçÈÎéÌðäÍíÖ2ÍÅûÞ7rÐê¡äßêX»ÞòNpñðÃfÂ_÷¾ÜÀ»(Î
ôþç6ðVοéq~ÿӁÎßÞÂ;Ëèš[÷Ý¡'QÒZfr¢³¥Ü—Çïnb¾TÒï³Ã¯êgâìîw}§Äìˆsg
Á"ΐKí#¯2ôÄdžl	́8ó7&䜐½~ôY]à^АϸS~?øø߂8''"¼=YÈ£=äȱeÝ:[Ê>Ç;(æ˜@ßqà¼Ð#˜Ղ¸Ÿë2RZ˜ä¡`­7÷Æk5~c6€Ü!âàâÑ{}—ЙA,´ÎKÕ2@#{øûìÅæÞؙ¾ã¬ØÅå±ÄÖž¹¾'è!¦‡5Ä~ǾW軼‹bNÐYAŒàŽÐÿ7ðcZ{z(_Wù7öýµ	ô.[x·Ü{Oª½EmCxHó–}urº1.òàåO×Ù@"ÃÄÀsUï
˜@ÿŅڐ;B-<}Ù}6ЃiÆÞ¯Í9Bö¿šÀݵð*¹Qr6×ølz_ôÕ£iäsï=QS,Qã$\{À30!÷ƒÆš,ÐÃޚèÝÖ:ÖæaHÎüTáfÉ=çÍC3÷¶5ÐCLÍ~Zõ"üx˜ê'gÿè!ž‡Ýz›?éÁŸ‡œy´å'þnFÞÕ{ÈՋ9–:2æOxè[+=øò+—!9æî=øñ`]?zðu_YÃî™}k¦‡z<Œµ®9g
­{IÃΈ¾5ÓC^¹<ìr""¡kz(äaNŽÖµ£‡2çCZ×Ò{šbxH掮ï]«‡5žã¡/×¾¦ßÑõû~—£žÖ}­Íûh=­ó¨ÅCz¤¹vå졟Q=ävÃØÜÛÖ0§}5¡ßJœ¹¾#¢‡RFæx(etÉuÑÃ:<]=Ð=¬ÓÐ5ÒÃtò|8CkhÝˈž/ô¾éÑM"X²ÛçÝô¿çC{èZ›u/éÁÇÞ§‡q'çCzèZ+=ó°çùÐæì‹QzÏÐC¬ÈU‡ÏW塹vë^z31ð»Â{ØW?ë>zò0"ªóP["¨OÍÒu×èdÁ:VãaŸ'ÖÝz z gªð`Ý/z°ëу¯°îQ…B{Xƒ	z 
z Âz°î=øëžÑƒ¯°î™‡ º : Z ú06ƃu<=Äð`]£µx°îóJM¸õɄujô`ÝSñáÁºo+í»['­X×g-¬ûL~<X÷xÅ\zˆæ¢2n<X÷"&|yˆèúFKx°®1ûçËC‰°v@s"<0ƒÑÿ®¶p
endstream
endobj
74 0 obj
<</BitsPerComponent 8/ColorSpace/DeviceGray/DecodeParms<</BitsPerComponent 4/Colors 1/Columns 132>>/Filter/FlateDecode/Height 134/Intent/RelativeColorimetric/Length 100/Name/X/Subtype/Image/Type/XObject/Width 132>>stream
H‰ìÎ1
°ù7
	&ÆÑ*h™6‡ú7VyÚÃÀ
endstream
endobj
73 0 obj
<</BitsPerComponent 8/ColorSpace/DeviceGray/DecodeParms<</BitsPerComponent 4/Colors 1/Columns 132>>/Filter/FlateDecode/Height 134/Intent/RelativeColorimetric/Length 100/Name/X/Subtype/Image/Type/XObject/Width 132>>stream
H‰ìÎ1
°ù7
	&ÆÑ*h™6‡ú7VyÚÃÀ
endstream
endobj
72 0 obj
<</BitsPerComponent 8/ColorSpace/DeviceGray/DecodeParms<</BitsPerComponent 4/Colors 1/Columns 154>>/Filter/FlateDecode/Height 133/Intent/RelativeColorimetric/Length 150/Name/X/Subtype/Image/Type/XObject/Width 154>>stream
H‰ìα
À À0þv&ÂRÙx®Ìm³fYg֙ufYg֙ufYg֙ufYg֙ufYg֙ufYg֙ufYg֙ufYg֙ufYg֙ufYg֙ufYg֙ufYg֙ufYg֙ufYg֙ufYg֙ufY÷ǏXÉ£Àß
endstream
endobj
71 0 obj
<</BitsPerComponent 8/ColorSpace/DeviceGray/DecodeParms<</BitsPerComponent 4/Colors 1/Columns 155>>/Filter/FlateDecode/Height 134/Intent/RelativeColorimetric/Length 151/Name/X/Subtype/Image/Type/XObject/Width 155>>stream
H‰ìα	 À0ÿZw'.'$dªùØQ»¢V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨jÅ¡Æ7–Fh
endstream
endobj
70 0 obj
<</BitsPerComponent 8/ColorSpace/DeviceGray/DecodeParms<</BitsPerComponent 4/Colors 1/Columns 155>>/Filter/FlateDecode/Height 134/Intent/RelativeColorimetric/Length 151/Name/X/Subtype/Image/Type/XObject/Width 155>>stream
H‰ìα	 À0ÿZw'.'$dªùØQ»¢V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨jÅ¡Æ7–Fh
endstream
endobj
48 0 obj
[/Indexed/DeviceCMYK 142 75 0 R]
endobj
69 0 obj
<</BitsPerComponent 8/ColorSpace/DeviceGray/DecodeParms<</BitsPerComponent 4/Colors 1/Columns 155>>/Filter/FlateDecode/Height 134/Intent/RelativeColorimetric/Length 151/Name/X/Subtype/Image/Type/XObject/Width 155>>stream
H‰ìα	 À0ÿZwA.'$dªùÚQ»¢V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨j…Z¡V¨jŹÆ7–7Gu
endstream
endobj
75 0 obj
<</Length 572>>stream
æô!æñæåæáæÄP+åÿ(
åÿ%	åü$åù!åîåéåÜ!åØ#åÕ#äÿ)ãÏ%ãË'ãÇ(âÿ,âÂ*áÿ/á¾*áº-	àÿ1à³0
à¯1
àª3ߥ6Þÿ5Þ 9ޛ;
ݗ<ݒ>
݆_#Üÿ7!܍A
ÛÿFGۈDۃFÚÿ8%ÙIØÿ;+ØzLØxMØsPØoR×ÿ=/Öÿ>5ÖkUÖgXÖbZÖ[nÕ^]Ôÿ>:ÔZ`
ÔVc
ÔTdÓQgÓMjÓIl
ÓDw
ÒEp	Ò=yÑÿ@AÑBs	Ñ?vÑ;~Ñ;zÑ:{ÐÿAGÐ:€Ð7}Ï3'Ï/"Ï,ˆÏ(Î%ÍÿCMÍ#'Ì •Ì–ËÿDTÊÿEZʝʞÈÿE[ȣȤǩƩĮðÁµÀ¶¿­«æ¾º¼»º¿·ÂµÄ²Ç¯É¬Ë©Î§Ñ¤Õ¢×ŸÛœÞ˜ã•æ'çŽìŠñ†õ'ü~ÿzÿuÿr
ìpÿlÿgÿbÿ\ÿXÿSÿNÿHÿCÿ<ÿ9ÿ7ÿ2ÿ,ÿ%ÿÿÿÿÿÿ	ÿÿ
endstream
endobj
68 0 obj
<</I false/K false/S/Transparency/Type/Group>>
endobj
49 0 obj
<</AIS false/BM/Normal/CA 1.0/OP false/OPM 1/SA true/SMask/None/Type/ExtGState/ca 1.0/op false>>
endobj
65 0 obj
<</I false/K false/S/Transparency/Type/Group>>
endobj
67 0 obj
<</BitsPerComponent 8/ColorSpace 66 0 R/Decode[0.0 255.0]/Filter/FlateDecode/Height 28/Intent/RelativeColorimetric/Length 94/Name/X/Subtype/Image/Type/XObject/Width 32>>stream
H‰"ÑI€ CQQ1èýLQ¸i†üÞ¾ÐA'ùì@ -(àfA¿Á¹ã®oÈàP•-Ɩ_ðiÁøM¸€c`ÁèF°RçkçòÇÿÀ
n¸,£OSd¼
endstream
endobj
66 0 obj
[/Indexed/DeviceCMYK 10 76 0 R]
endobj
76 0 obj
<</Length 44>>stream
ìùI.äµR)ä³S)ÚÿFIÚsf×amÖÿDNÒ=yÌÿEXÊÿEZÈÿE[
endstream
endobj
56 0 obj
<</Color[20224 32768 65535]/Dimmed false/Editable true/Preview true/Printed true/Title(Calque 1)/Visible true>>
endobj
52 0 obj
<</BaseFont/QENXPK+LMRoman10-Regular/Encoding/WinAnsiEncoding/FirstChar 32/FontDescriptor 77 0 R/LastChar 215/Subtype/Type1/Type/Font/Widths[333 0 0 0 0 0 0 0 389 389 500 0 0 333 0 0 0 500 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 778]>>
endobj
53 0 obj
<</BaseFont/QENXPK+LMRoman10-Bold/Encoding/WinAnsiEncoding/FirstChar 32/FontDescriptor 78 0 R/LastChar 120/Subtype/Type1/Type/Font/Widths[383 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 607]>>
endobj
54 0 obj
<</BaseFont/QENXPK+LMRoman10-Italic/Encoding/WinAnsiEncoding/FirstChar 104/FontDescriptor 79 0 R/LastChar 104/Subtype/Type1/Type/Font/Widths[511]>>
endobj
55 0 obj
<</BaseFont/QENXPK+LMSans10-Regular/Encoding/WinAnsiEncoding/FirstChar 32/FontDescriptor 80 0 R/LastChar 118/Subtype/Type1/Type/Font/Widths[333 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 667 0 639 0 0 0 0 0 278 0 0 542 875 0 736 0 0 646 0 0 688 0 0 0 0 0 0 0 0 0 0 0 481 0 444 517 444 306 500 0 239 0 0 239 794 517 500 517 0 342 383 361 517 461]>>
endobj
80 0 obj
<</Ascent 1154/CapHeight 694/CharSet(/space/A/C/I/L/M/O/R/U/a/c/d/e/f/g/i/l/m/n/o/p/r/s/t/u/v)/Descent -309/Flags 32/FontBBox[-420 -309 1431 1154]/FontFamily(LM Sans 10)/FontFile3 81 0 R/FontName/QENXPK+LMSans10-Regular/FontStretch/Normal/FontWeight 400/ItalicAngle 0/StemV 76/Type/FontDescriptor/XHeight 444>>
endobj
81 0 obj
<</Filter/FlateDecode/Length 2105/Subtype/Type1C>>stream
H‰\TkPWîf¦»qTÆ'f»[Ĉޛ¨v'gñ‡€B\^300030²Šâ">ßQÄ⥥³hy9
²8.!>ÐÕÔXOSj·ÇlåÇVwÝ®¾ç|_ûï\[a8ŽÛGEÆ)—G¬NÎÖyz¸~®LÏËJÖZbÎ<óŽbþ¶²©•èŽ#qÜQü7L³áíx7×äh]b‡‰püþðx€&§@«NÏÐs^Þ[֕œ¿–œš©1è2Õ\rvæÆ­uã"5aW͹h²¹eFr–ŠÓ¨¸e—§Sju\ºV"—£[êÆÅd¨uœA£Í䄯V™¥LÖ)Ó¸¼ì4¥–Óg(¹õÑ1\°&[ÏE¨S•Ù:%çêÊq:¥'ËÐës|ÜÝõyénmº»JÈѹgý–¤s·à\ƒ×EƸF"EF¹é7ë9•FË¥)õÉê,[¤FûUr–{ptLAŽ'óô*ÅsÂ0g[†a®8æaÞö)†ùcX ðµb,ZŒa-ˆ‹‰0S`UX3֋/Ãwà}V6VYVM¢™¢dQ•xƒø¯ââDŽ"ø'h"†É²˜l%'B%Û$0T"I|°?ÿMÚÉQÅdáM¢Šé0bˆ|I\%GP±Êehy©œ"¥¦ûÜ£#ÍÖûÈý…G´u¡Öø{^ÿ¾ïñe%÷‰¸€M;'i´Ü>WX1NÀ>¼¦Í¹ÂVŽõëËBiƒh´Å¡õ°BìØ¥ò–VR"?fÀ_Ž‹ \>æ5FI ÎØ3ióa"ß-¿G¡ê½Dü¤#%üéßoÌ|¥Y4Y)`I!9úw†GšS"° "ÜU³½yëäÉ{Ù«Ÿˆ˜3ObûÈٗ~:\¦Øÿ""ðöH}Ó0x¨nÁ¾Rb£$¼C^/ÿkÞ1ÎG‹&WÄTh1|'|ПZÒP¸ wX«a1x'Šñª"¡X"!	"'̅+ÀAÖïB	´	Ú÷› ¼õŽŠøi9Š‡‡Ä»³}£¯þ-bPÉtØcè/¨Ÿ0ð‡dá
dà g(g¬ï)Y	ü"×1ébQ™Eü3("ñɾS)²_ºbÕª»@3|Š×T2…>'€*Z,B™À¹
Ü»ñ«ƒ/̍~'®P¿ø÷»‡mڒ"À%šo~_~n½œº†M¢Ð²½HšìíÔàó¤âåþﺘtjØË6µêÍLA¶²´ˆÞ¸©îJ?|z¤e?+™(ꁟ{ð&Ùû²¬¤H[_G¯Œœ07¿úõfcqz;{¼—hT¨F҈õA³
šó\¨sî­öŠæ[¬¤ÈtÆ	¦ìšÌ°Ëì7,]Ê­öC­"tøê†è2íâ»ÉÐü‹ºÐ}ôVK+.,-ÈÌfzmq.½Ö¿æ€ýão»YiÊwgõ™µ–òLàÛv&üâ0;E¼hd¥Ãi·™;)'eé4y.hí_9íÝÎú3—Ø'^"6"t·ž^>0±‡…Cí2d$GN´}ßIßìP»—³'Ôš|^Þ%Ԍ¿Á›IJÖG؞õµŠv
\Âz®‰š'ór°êB̤†úŽœ®nØ»µQèˆJ鄏owBF§Ý™þô~é¯î—ÎãxGYÑ]"(jó¶¯Øª|ue*ý‰€‡ª<½:—ÍN1¦írÈ=š]•ÏH_ÅfmOÌuð{½$0ûu÷`ÑjcãMnÛdl+;xâÈQvkͅÂfúYÿÐøµ¼æ¢Jö`)Q{æ`=}òÛ=Fù/'ù&h'i™*¶nlìf]sK«Æ—}6…Éþüå*Fêx®õ€±×Ì>#k0³N8´ÂNãvÃã+‡¥&ðó
¿)%õãïÊƽ¼(KŽeXGU<,í³L7#>j†–wÞÊÉD9Ü ú¶<C³ÖÅjÖ«˜'ܠÙt@BJz;0µÁ{©4Œ½8¦dÐÕÿû¥$¿Æ¶±ÝÛúI<ãCŠK˜ÿÜ;56òj_`æ¸	>}cÂϚÁbU5äÈÀaÉ{4Í^†¬Ð|dÿ‹ÌÛ7oAÎø"!›Śà€˜³F®÷öÆ
s)Akò!Ü/{ð,6ñzÐÉÀ6ÄË×Eå§%2×ý¦íÌ°"Ê>wUs›þùé8²¾rçÀ ¿´œê³£Ò¸ÿ¤$Rë/ÕµÐ#·ÿìÎJvÇÙhÀDûo/XÉ«4&>+ÑúyÐԆaø'z388±Ÿ'4݅wÝø…X; ')˜'kW5î=À¤]Ì9üÅQ똲Äc×îËÏ·íVw2ÂÌÕǦ|GkÑB#šÿMæ©Íì¹¼ÚÝíEÖM;»¶opþ̸Õ'ºùx³="Ør¾]3JŸl7žoaÏÕW]nqT
'=î©7('G
²-ÝD~næöLZUx¶…°°-i0'þ1êGTM­«ºßãTù)FRÔÎ;ìFÍF3ؚ¥"&ñ
_ÔBùEg"î<ÝÂÀ"ô…/zJÔmk8ÑrÙ(´‰ú`2¼'ñŸó
™ùJˏÉò)¶\ô%M¹÷w4,ƒãö¾$Ö#ž''¼Z^Q±µ'jI¦&(Ãÿc;Ãh;Óô_qÝäÞ<«zû€hÏ©I½}} >ËÃûc¦È÷w¢bþ
endstream
endobj
79 0 obj
<</Ascent 1125/CapHeight 683/CharSet(/h)/Descent -290/Flags 98/FontBBox[-458 -290 1386 1125]/FontFamily(LM Roman 10)/FontFile3 82 0 R/FontName/QENXPK+LMRoman10-Italic/FontStretch/Normal/FontWeight 400/ItalicAngle -15/StemV 68/Type/FontDescriptor/XHeight 442>>
endobj
82 0 obj
<</Filter/FlateDecode/Length 568/Subtype/Type1C>>stream
H‰bd`ab`dd"tõ‹ðÖöñ
ÊÏMÌ34Ðõ,IÌÉLÉiþfü!Ã"÷Ћ9é?ÓYÑ?q¿·É°fýúÉúý,À÷'‡ô1032^¸öÄ9¿ ²(3=£DÁÈÀÀXDZ(8é)x%&gç—gg*$æ¥(xé)øê)øå—E34òó'R3sÒòÓBR#J‹S‹ŠҋòKŠ5õB22‹Êó‹²€tQjNjbqjŠBi^Jj'BIFª'{hpˆ'[~^‰'Ofrj^qª'®®'BqjªBFII•¾~Iiº^~Qº~PM±~DQ±>HŸ®›¿_ˆ®§³«_°«^IE‰BZ~'BJjIbfN±ž_~QnbŽ¾[pHeAª'¡P"<˜Y¶_Ã÷crú¿§meüþàðÜÌ?VWÚÜÝR×ÝYÓ.WÐ\ (]Ö5k撩K'/–Ÿ`Ëw–£RwCFyddäæÈ]ù¾ƒµ§¯wj·Ô"Ö¾æŽÆ®®9fÖú®†®
©†©Ý3w÷¶4vtÔvËýÖø󈵫³«¡[ªaJͼ3æLë"ÛöÝq‰&,"œ²¾§wîjŽÕ󷝺(½½7®Ì7þ7wm²|]fGS™TüòôÝ/Ö~ל ÇWºð‡ó´ïŽ³²É-puc`üÏÃÙÍýë0÷¾žÞޞþžþM&òðlœÛß3©§gfτy?ððÝßP
endstream
endobj
78 0 obj
<</Ascent 1133/CapHeight 686/CharSet(/space/x)/Descent -295/Flags 34/FontBBox[-486 -295 1607 1133]/FontFamily(LM Roman 10)/FontFile3 83 0 R/FontName/QENXPK+LMRoman10-Bold/FontStretch/Normal/FontWeight 700/ItalicAngle 0/StemV 108/Type/FontDescriptor/XHeight 444>>
endobj
83 0 obj
<</Filter/FlateDecode/Length 492/Subtype/Type1C>>stream
H‰$‹OhÓpÅó뚆¹¬þ¯B‹û''MÒ̓"ž6Ûáìê´&+B\~mC»üJ~)mwTڑ.ÚV»í6ïó$^"x²ëðî®^<ÍÃ/A3|‡÷àóÞC\8Ä!"bRÙ¥Å×3ÉªjL%¥RՎ›Ë^yçÂ^B<ÿgÍÿ'ˆÌ%«<ûz'íbßNïyÙ3\¡ƒÃYRk™z©lÁt2yóƱ߆æՕ
iЊª¡Á¼2dI# :\#<ÇeµZR"<^':Å&…'Iê5:)C¾¬Sh³Aš¸ŠUŠ5¨6Á*c˜{'ËCšdôlP'@1†²eÕî(ŠU/ÉÄ,)Å`C•êÿUŽRúa6/eîϦ²¹"l5-(4l©z•ÊJ:—oÕ0LM¨ÈBÜÓÀG
/ÙnÔ;õ~Û.;rÑoÄûsï	þ]¶ÌFYŒßÞêõã® t®8|AØÞ\µ9Ñ~m¯·Û·¤‹"Là?¹¼ã‡'ú»À'~Æ¿à_å›k%{9^~:GÞZÍ·=ÛÞè&~1ÄB~Œ×
&:|ôÅÐ[|Ǟí¼F.í¤Òú+ŽÚâ˜{'EÆv§ÛÝxÓí÷?Ûû¼ÕsΠ7tÄñˆg·
endstream
endobj
77 0 obj
<</Ascent 1127/CapHeight 683/CharSet(/space/parenleft/parenright/asterisk/hyphen/one/multiply)/Descent -290/Flags 34/FontBBox[-430 -290 1417 1127]/FontFamily(LM Roman 10)/FontFile3 84 0 R/FontName/QENXPK+LMRoman10-Regular/FontStretch/Normal/FontWeight 400/ItalicAngle 0/StemV 68/Type/FontDescriptor/XHeight 431>>
endobj
84 0 obj
<</Filter/FlateDecode/Length 878/Subtype/Type1C>>stream
H‰<P_lu¿Ûí¨°®ûƒEÚâÝŸ Òve1¨Ñ™l®dcë6Ö%[*»þIK¯Þ]éÆÚkOÖ´Í­×u㺻2¢$d1³à£&Ɖy'èJ$ñEãƒÉïàG¢7Mü>|¿ù~þ%ß/Žµ·a8Ž;¦†³"§^?͞
§|}îÓL4"s»äk†7µ¯Zí/ї‡ÈêsD»]ðQ7ü±çÞ³Ÿ{1Ç>úuˆM/rñhLÇûúúíö7Á Œ†Ï$Ø,ŸˆƒpjŒzÀ¸ج‰ÆÁ6>dbád°dfA†g8D96"æz@0çA–åÀœ"dÂ<32©y†BŒ'g¦ƒÀϦ0?äx¸Ýðb'~Ûë2QËE½SÃ{"ÿ‰xï®ÏíŸÝc#CÁéa° €ˁyFǓ¼'ÀrgÃI¯:¸˜f€ï¸ID0³pl/¶ëÀlX/vÃÜ_2_ˆ‰}€mãïà"¸Šÿl3¶Z<÷<—ÅÿØ!àc´lWäÚùM
õÀÞœ'n'üÂ.ØCirMq®••'ä;‰öOR³¨­€ˆÎw›¨óDR¨ëî/£ª«QWÖèÿsá'|*öŸŠ°3I
vM¼q_r•ÊåRE®^Y¤?ò-êGŒ½Aï£nÔK‰¹Zq–êå†úô{¸ÿõlۀÄc§
þvÎÊâ÷
'0üƸ½Y^?¿N¡Ã ý€¼r±¾¶áԊ­¥åª¼ð…ˆ·Zp€l‰ª¸T,ˆT
 î§d3_•K®¥bN,Ö/l^ ááD——NYf?§ ø3‡Ȝ&i—š•ƒðÀ1²²ªTÖ]—š-¶ÍÀ‰¼	/ðœ°ï ËS›¼eÜÚúÎ<9ýaœ8°•°ø*Í[´±cùT®	Ô©ñ~9áJZ>¹#_ÿš~ѲD+•HîQn>'·]ÛOäÊMÚf¸žµ·ìº.j'ŠB0tÎÁªêZ^wätQ"$4‡æîR'*j¹¼#Ÿ×óªC(d¢($IyQÏ;ZyMSUøo'‰ª'&êºÃ–¹fmÂT³qmuu؏á[÷Ê֎­};®®¬ÔVjµ•‹5åžÕúÙªz]Yo4"ÕFÝÚiT^6^±ÿ#ÀM@~Ö
endstream
endobj
50 0 obj
<</AIS false/BM/Normal/CA 0.779999/OP false/OPM 1/SA true/SMask/None/Type/ExtGState/ca 0.779999/op false>>
endobj
51 0 obj
<</AIS false/BM/Normal/CA 0.800003/OP false/OPM 1/SA true/SMask/None/Type/ExtGState/ca 0.800003/op false>>
endobj
85 0 obj
<</CreationDate(D:20160201152316+01'00')/Creator(Adobe Illustrator CC 2015 \(Macintosh\))/ModDate(D:20160201152445+01'00')/Producer(Adobe PDF library 10.01)/Title(Impression)>>
endobj
xref
0 86
0000000004 65535 f
0000000016 00000 n
0000000076 00000 n
0000061744 00000 n
0000000000 00000 f
0000061795 00000 n
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000062319 00000 n
0000064022 00000 n
0000104138 00000 n
0000105272 00000 n
0000113036 00000 n
0000113159 00000 n
0000106015 00000 n
0000106557 00000 n
0000106896 00000 n
0000107060 00000 n
0000105887 00000 n
0000064088 00000 n
0000064416 00000 n
0000064650 00000 n
0000065600 00000 n
0000074599 00000 n
0000083734 00000 n
0000089626 00000 n
0000097545 00000 n
0000105385 00000 n
0000105746 00000 n
0000105448 00000 n
0000105209 00000 n
0000104187 00000 n
0000103738 00000 n
0000103338 00000 n
0000102939 00000 n
0000102590 00000 n
0000102241 00000 n
0000104587 00000 n
0000105794 00000 n
0000111745 00000 n
0000110890 00000 n
0000109962 00000 n
0000107445 00000 n
0000107772 00000 n
0000110238 00000 n
0000111169 00000 n
0000112074 00000 n
0000113282 00000 n
trailer
<</Size 86/Root 1 0 R/Info 85 0 R/ID[<2CFE353CC5884793AE8343ADBDA0D3FF><BCCE9EABF98A47668DFB74F0D7E2D7D0>]>>
startxref
113475
%%EOF

